Easy, Interpretable, Effective: openSMILE for voice deepfake detection

In this paper, we demonstrate that attacks in the latest ASVspoof5 dataset -- a de facto standard in the field of voice authenticity and deepfake detection -- can be identified with surprising accuracy using a small subset of very simplistic features. These are derived from the openSMILE library, and are scalar-valued, easy to compute, and human interpretable. For example, attack A10`s unvoiced segments have a mean length of 0.09 +- 0.02, while bona fide instances have a mean length of 0.18 +- 0.07. Using this feature alone, a threshold classifier achieves an Equal Error Rate (EER) of 10.3% for attack A10. Similarly, across all attacks, we achieve up to 0.8% EER, with an overall EER of 15.7 +- 6.0%. We explore the generalization capabilities of these features and find that some of them transfer effectively between attacks, primarily when the attacks originate from similar Text-to-Speech (TTS) architectures. This finding may indicate that voice anti-spoofing is, in part, a problem of identifying and remembering signatures or fingerprints of individual TTS systems. This allows to better understand anti-spoofing models and their challenges in real-world application.

==> tex/contributions.tex <==
\dan{
Contributions (mostly similar to those identified by Nicolas in the abstract, but with a bit more focus on the general problem, that is, not specific to ASV5; edit: I think Nicolas' story, focusing on ASV5, makes more sense):
\begin{enumerate}
    \item  We build explainable deepfake detection models by leveraging human-interpretable features from OpenSmile.
    \item These features are highly predictive in-domain, when training and testing on audios produced by the same attack.
    The results are strong even with a simple logistic classifier, which preserves explainability.
    \item However, the performance of these features degrades out-of-domain.
    The level of degradation depends on the type of attacks;
    for ASV5 we observe that attacks in train are very similar among themselves and
    different from those in the validation split.
\end{enumerate}
%
Comments:
\begin{itemize}
    \item Why do we observe this pattern of generalization in ASV5?
    Hard to tell without access to more metadata.
    Should we listen to some audios?
    Alternatively, we could consider ASV19 for which we have information about the attacks.
    This extra information might allow us to draw more sensible conclusions,
    but the extra work involved makes this direction more suitable for a next submission.
    \item I don't have a good claim pertaining to wav2vec features.
    Wav2vec features show some similar patterns of generalization to hand-crafted features,
    but only if we restrict ourselves to a \textit{single} feature.
    But this setup is not typically used in practice, so I find this experiment a bit hard to motivate.
    \item (2024-07-17 09:40)
    Even for openSmile features it may not be immediately clear why we restrict ourselves to using a single feature.
    I think Nicolas' original motivation was to identify shortcuts (spurious features).
    I don't know we should be explicit about this aspect.
    (Edit: I see that Nicolas was explicit about this in the abstract)
    \item (2024-07-17 09:40)
    Some of the features in openSmile are not that easily interpretable (for example, F749 in the \texttt{emobase} set refers to ``simple moving average of MFCC 12 - linear regression coeff A'').
    We might need to address this at some point in the paper.
    \octav{Maybe we should not include emobase results. Overall emobase contains harder to understand features, and eGeMAPS should be enough to articulate our arguments.}
    \item If Horia is unconfortable with the fact that wav2vec was trained on Multilingual LibriSpeech,
    we could use a variant trained on LibriSpeech only, for example, \texttt{wav2vec2-large} or \texttt{wavlm-large} (instead of the \texttt{wav2vec2-xls-r-2b} that was used by Octav).
    \item (2024-07-17 10:00)
    Some comments regarding the current version of the abstract:
    \begin{itemize}
        \item ``easy to compute'' → ``efficient to compute''? It's not complicated to extract wav2vec features :-)
        \item "binary behavior" → isn't this claim too strong? I see values all over the [0--50] range in Octav's matrices;
        I would expect narrower distributions when reading this claim.
        \item ``pretrained front-ends rely on a small set of characterstics'' → which experiment supports this claim?
        \item ``generalization capability'' → note that for the single-feature experiments we are using a more lenient scenario in which we train the classifier on the \textit{target} attack
        (maybe this is not as bad as I first thought, because we have a single feature and use a threshold-free metric; so this affects only those cases when the classifier changes the sign of the weight between attacks).
        We should also prepare the 8 (train) $\times$ 16 (train + validation) matrices.
        \end{itemize}
\end{itemize}
}

\octav{
Contributions
\begin{itemize}
    \item We show that a simple LogReg model trained on hand-crafted features offers high-accuracy in-domain.
    \item We make a case that different attack types can have different predictive features for ASV5 
    \item We motivate that a deepfake classifier may rely on these shortcuts when learning which results in poor performance out-of-domain (train vs dev)
\end{itemize}
}

\dan{
Contributions (mostly similar to those identified by Nicolas in the abstract, but with a bit more focus on the general problem, that is, not specific to ASV5; edit: I think Nicolas' story, focusing on ASV5, makes more sense):
\begin{enumerate}
    \item  We build explainable deepfake detection models by leveraging human-interpretable features from OpenSmile.
    \item These features are highly predictive in-domain, when training and testing on audios produced by the same attack.
    The results are strong even with a simple logistic classifier, which preserves explainability.
    \item However, the performance of these features degrades out-of-domain.
    The level of degradation depends on the type of attacks;
    for ASV5 we observe that attacks in train are very similar among themselves and
    different from those in the validation split.
\end{enumerate}
%
Comments:
\begin{itemize}
    \item Why do we observe this pattern of generalization in ASV5?
    Hard to tell without access to more metadata.
    Should we listen to some audios?
    Alternatively, we could consider ASV19 for which we have information about the attacks.
    This extra information might allow us to draw more sensible conclusions,
    but the extra work involved makes this direction more suitable for a next submission.
    \item I don't have a good claim pertaining to wav2vec features.
    Wav2vec features show some similar patterns of generalization to hand-crafted features,
    but only if we restrict ourselves to a \textit{single} feature.
    But this setup is not typically used in practice, so I find this experiment a bit hard to motivate.
    \item (2024-07-17 09:40)
    Even for openSmile features it may not be immediately clear why we restrict ourselves to using a single feature.
    I think Nicolas' original motivation was to identify shortcuts (spurious features).
    I don't know we should be explicit about this aspect.
    (Edit: I see that Nicolas was explicit about this in the abstract)
    \item (2024-07-17 09:40)
    Some of the features in openSmile are not that easily interpretable (for example, F749 in the \texttt{emobase} set refers to ``simple moving average of MFCC 12 - linear regression coeff A'').
    We might need to address this at some point in the paper.
    \octav{Maybe we should not include emobase results. Overall emobase contains harder to understand features, and eGeMAPS should be enough to articulate our arguments.}
    \item If Horia is unconfortable with the fact that wav2vec was trained on Multilingual LibriSpeech,
    we could use a variant trained on LibriSpeech only, for example, \texttt{wav2vec2-large} or \texttt{wavlm-large} (instead of the \texttt{wav2vec2-xls-r-2b} that was used by Octav).
    \item (2024-07-17 10:00)
    Some comments regarding the current version of the abstract:
    \begin{itemize}
        \item ``easy to compute'' → ``efficient to compute''? It's not complicated to extract wav2vec features :-)
        \item "binary behavior" → isn't this claim too strong? I see values all over the [0--50] range in Octav's matrices;
        I would expect narrower distributions when reading this claim.
        \item ``pretrained front-ends rely on a small set of characterstics'' → which experiment supports this claim?
        \item ``generalization capability'' → note that for the single-feature experiments we are using a more lenient scenario in which we train the classifier on the \textit{target} attack
        (maybe this is not as bad as I first thought, because we have a single feature and use a threshold-free metric; so this affects only those cases when the classifier changes the sign of the weight between attacks).
        We should also prepare the 8 (train) $\times$ 16 (train + validation) matrices.
        \end{itemize}
\end{itemize}
}

\octav{
Contributions
\begin{itemize}
    \item We show that a simple LogReg model trained on hand-crafted features offers high-accuracy in-domain.
    \item We make a case that different attack types can have different predictive features for ASV5 
    \item We motivate that a deepfake classifier may rely on these shortcuts when learning which results in poor performance out-of-domain (train vs dev)
\end{itemize}
}


\nico{
Contributions
\begin{itemize}
    \item We demonstrate that only a few openSmile features are sufficient to identify ASV5 attacks with high accuracy.
    \item We show that the generalization of these features is strong but limited to certain attacks. This suggests that voice deepfake detection may operate similarly to antivirus signatures by identifying highly specific characteristics for each attack.
    \item We compare the openSmile feature set with features from a Wav2Vec2 (W2V2) front-end and show that there are similarities in terms of in-domain and out-of-domain generalization, as well as the number of predictive, scalar features.
\end{itemize}


% \begin{itemize}
%     \item Show that very few openSmile fatures suffice to identify ASV5 attacks.
%     \item Show that generalization of these features holds only for some attacks, but there, strongly. This may indicate that voice deepfake detection might operate similar to anti-virus signatures, i.e. identify highly specific characterics per attack.
%     \item We compare the openSmile feature set with features from a W2V2 front-end and show that there exist similarities regarding in- and out-of-domain generalization, as well as the quantity of predictive, scalar features.
%%%%%%%%%%%%%%%%%%%%%
    % \item Build XAI usin OpenSmile and show that some features (eg. zeroCrossingRate) are very predictive, i.e. are distributed differently for spoof and bona-fide (see Fig1)
    % \item Use these feats to explain attacks in ASV5. Observe different behaviour in train and dev partition: Similar features and good generalization in train; very different features per attack in dev, consequently poor generalization
    % \item Can show that using neural features (from W2V2) behave similarly: Similar features for attacks in train + good generelization; different feats and no gen. for dev
    % \item Extrapolate: Audio Deepfake detection not a homogeniuos task, generalization does depend on combination train/test attack. Also, show that openSmile can explain attacks and model behavior to some degree.
% \end{itemize}
}

\nico{
Contributions
\begin{itemize}
    \item We demonstrate that only a few openSmile features are sufficient to identify ASV5 attacks with high accuracy.
    \item We show that the generalization of these features is strong but limited to certain attacks. This suggests that voice deepfake detection may operate similarly to antivirus signatures by identifying highly specific characteristics for each attack.
    \item We compare the openSmile feature set with features from a Wav2Vec2 (W2V2) front-end and show that there are similarities in terms of in-domain and out-of-domain generalization, as well as the number of predictive, scalar features.
\end{itemize}
}

% Contributions (Nico)
% \begin{itemize}
%     \item Make attacks in ASV5 understandable by finding human-interpretable features that predict attack to high degree of accuracy
%     \item Analyze transferability of these features: Show that these features transfer very well within the \emph{train} set of ASV5, but not for \emph{dev} set of ASV5
%     \item Show that large-pre trained models such as W2V2 extract similar features as the ones we found,
%     \item Conclusion:
% \end{itemize}


==> tex/results/expA.tex <==
% \subsection{Results Experiment A}\label{sec:resA}

Consider \Cref{tab:expA}, which presents the results for in-domain evaluation.
For most attacks, a single openSMILE feature is sufficient to achieve good performance, with results as low as $0.8\%$ EER for attack $A14$. The worst performance is observed for attack $A16$, where the best performing feature $F66$ yields an EER of $23.8\%$. 
% This is still relatively good, given the simplicity of the approach. 
On average, this simplistic approach achieves $16.3 \pm 6.3\%$ EER - much better than random guessing.

These results indicate that each attack has a distinctive fingerprint, and is characterized by unique, but simplistic patterns. 
While some attacks are more easily identified than others, this principle holds throughout ASVspoof5. 
Interestingly, certain features, such as $F17$, are effective across multiple attacks (7 out of 16 attacks), whereas others, like $F51$, are highly effective for specific attacks (e.g., $A14$ with $0.8\%$ EER) but not for others.
Some of the most occurring features in \Cref{tab:expA} are:
\begin{itemize}
\itemsep0em
    \item \textbf{F17 (7 occurrences):} loudness\_sma3\_stddevRisingSlope - standard deviation of the rising slope of the simple moving average (with a window size of 3) of the loudness.
    \item \textbf{F19 (7 occurrences):} loudness\_sma3\_stddevFallingSlope - standard deviation of the falling slope of the simple moving average (with a window size of 3) of the loudness.
    \item \textbf{F66 (6 occurrences):} spectralFluxV\_sma3nz\_amean - arithmetic mean of the simple moving average (with a window size of 3) of the spectral flux for non-zero values.
    % \item \textbf{F21 (3 occurrences):} spectralFlux\_sma3\_stddevNorm - standard deviation-normalized simple moving average (with a window size of 3) of the spectral flux
    % \item \textbf{F12 (2 occurrences):} loudness\_sma3\_percentile20.0 - the 20th percentile of the simple moving average of the loudness values over 3 values
    % \item \textbf{F20 (2 occurrences):} spectralFlux\_sma3\_amean - arithmetic mean of the simple moving average of spectral flux over a window of 3 values
    \item \textbf{F85 (2 occurrences):} MeanUnvoicedSegmentLength - average length of all unvoiced segments within the audio file.
    \item \textbf{F86 (2 occurrences):} StddevUnvoicedSegmentLength - standard deviation of the length of all unvoiced segments.
    % within the audio file.
\end{itemize}

\begin{table}[]
\centering
\caption{In-domain test performance per attack, for the top-3 features per attack $A01$ through $A16$.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\cline{1-3} \cline{5-7}
Attack & Feature & \multicolumn{1}{l|}{Test EER} &  & Attack & Feature & \multicolumn{1}{l|}{Test EER} \\ \cline{1-3} \cline{5-7} 
\multirow{3}{*}{A01} & F66 & 12.8 &  & \multirow{3}{*}{A09} & F86 &  8.0 \\ \cline{2-3} \cline{6-7} 
                     & F19 & 13.8 &  &                      & F85 & 11.5 \\ \cline{2-3} \cline{6-7} 
                     & F17 & 14.7 &  &                      & F12 & 12.7 \\ \cline{1-3} \cline{5-7} 
\multirow{3}{*}{A02} & F66 & 12.7 &  & \multirow{3}{*}{A10} & F86 &  7.3 \\ \cline{2-3} \cline{6-7} 
                     & F19 & 13.0 &  &                      & F85 & 10.7 \\ \cline{2-3} \cline{6-7} 
                     & F17 & 13.6 &  &                      & F12 & 12.2 \\ \cline{1-3} \cline{5-7} 
\multirow{3}{*}{A03} & F19 & 15.3 &  & \multirow{3}{*}{A11} & F58 & 15.3 \\ \cline{2-3} \cline{6-7} 
                     & F66 & 15.7 &  &                      & F60 & 15.3 \\ \cline{2-3} \cline{6-7} 
                     & F17 & 15.8 &  &                      & F59 & 17.7 \\ \cline{1-3} \cline{5-7} 
\multirow{3}{*}{A04} & F19 & 16.8 &  & \multirow{3}{*}{A12} & F82 & 18.2 \\ \cline{2-3} \cline{6-7} 
                     & F21 & 17.3 &  &                      & F19 & 21.3 \\ \cline{2-3} \cline{6-7} 
                     & F81 & 20.1 &  &                      & F83 & 22.8 \\ \cline{1-3} \cline{5-7} 
\multirow{3}{*}{A05} & F21 & 17.5 &  & \multirow{3}{*}{A13} & F67 & 22.1 \\ \cline{2-3} \cline{6-7} 
                     & F19 & 19.4 &  &                      & F39 & 22.8 \\ \cline{2-3} \cline{6-7} 
                     & F17 & 20.0 &  &                      & F49 & 25.0 \\ \cline{1-3} \cline{5-7} 
\multirow{3}{*}{A06} & F21 & 16.8 &  & \multirow{3}{*}{A14} & F45 &  0.8 \\ \cline{2-3} \cline{6-7} 
                     & F19 & 17.1 &  &                      & F51 &  0.8 \\ \cline{2-3} \cline{6-7} 
                     & F17 & 19.3 &  &                      & F57 &  0.8 \\ \cline{1-3} \cline{5-7} 
\multirow{3}{*}{A07} & F66 & 13.7 &  & \multirow{3}{*}{A15} & F78 & 20.7 \\ \cline{2-3} \cline{6-7} 
                     & F1  & 14.2 &  &                      & F77 & 25.7 \\ \cline{2-3} \cline{6-7} 
                     & F17 & 14.6 &  &                      & F76 & 26.8 \\ \cline{1-3} \cline{5-7} 
\multirow{3}{*}{A08} & F20 & 17.7 &  & \multirow{3}{*}{A16} & F66 & 23.8 \\ \cline{2-3} \cline{6-7} 
                     & F66 & 18.2 &  &                      & F18 & 26.8 \\ \cline{2-3} \cline{6-7} 
                     & F17 & 20.2 &  &                      & F20 & 27.3 \\ \cline{1-3} \cline{5-7} 
\end{tabular}%
}
\label{tab:expA}
\end{table}


%\begin{figure}
%    \centering
%    \includegraphics[width=0.9\linewidth]{figs/table_explanation.png}
%    \caption{Predictive Features and their interpretation}
%    \label{fig:predictive_feats}
%\end{figure}

% \input{tex/table_features_explained}

==> tex/results/expB.tex <==

% \subsection{Results Experiment B}\label{sec:resB}

% \todo[inline]{color scheme between tab1 and tab2 is different - do we want to unify? Octav: Maybe we shouldnt use color scheme at all for table 1. I think that we shouldn't use the color scheme from Table 2 because it would all be green anyway. Nico: Yes, good point. Let's remove the colorscheme for Table 1.}
% This section presents results of out-of-domain (OOD) evaluation, where we assess how well the features identified in Experiment A (in-domain setting) generalize to unseen attacks. 
The results are shown in \Cref{tab:expB}, where the rows indicate the training attack, and the columns indicate the evaluation attack.
% The diagonal indicates the in-domain performance and is thus identical to \Cref{tab:expA}.
Note that \Cref{tab:expB} can be partitioned into four sub-matrices based on the `train' and `dev' partitions of the ASVspoof 5 dataset.
Systems trained on attacks $A01$ through $A08$
%that perform well in an in-domain setting for attacks $A01$ through $A08$ (i.e., attacks from the `train' partition) 
generalize relatively well to other `train' attacks, as indicated by the green highlights and correspondingly lower EERs ($19.7 \pm 6.9$\%) in the top-left quadrant. 
Some systems trained on the `dev' split exhibit good generalization to other `dev' attacks, e.g., $A09$ to $A10$.
When analyzing the attacks and their respective underlying TTS algorithms, c.f. \Cref{tab:attack_desc}, we observe that this behavior can be partially attributed to similarities in the TTS architecture used.
For instance, both $A09$ and $A10$ are derived from ToucanTTS\cite{lux2022low}, and thus generalize well between themselves.
Similarly, $A01$, $A02$, and $A03$ originate from a GlowTTS architecture \cite{kim2020glow}, which accounts for the observed strong generalization among them.
Generalization across different TTS architectures often proves challenging; for example, systems trained on $A16$ do not generalize to any of the attacks from $A01$ through $A08$.


In summary, generalization from `dev' to `train' and vice-versa is challenging, as indicated by the predominantly red highlights and high EERs ($53.5 \pm 16.5$\%) in the bottom-left and top-right quadrants.


%While there are some exceptions, %such as feature $F21$ from attack $A07$ transferring to attack $A09$ with an EER of about $18.1\%$, 
%most of the distributions are too different for the linear regressor to transfer effectively.

% NICO: NOT SURE IF THE FOLLOWING IS NECESSARY
% It is important to note that both front-end and back-end are derived from the initial in-domain training data.
% Thus, poor performance in the OOD setting may not necessarily indicate that the feature in question is unsuitable for cross-domain generalization. 
% Instead, it may suggest that the threshold learned by the linear regressor on the training data does not work well on the test data. 
% Particularly, when the EER is $> 50\%$, a better score could in theory be achieved by inverting the backend's output.
% This, however, is not practical, since the OOD test data is inaccessible for model training.
% This approach mirrors real-world environments, where both the feature (i.e., the front-end) and the learning model (i.e., the back-end) are derived solely from the training data.


%\begin{figure*}
%   \centering
%   \includegraphics[width=0.45\linewidth]{figs/expB/tab_train.png}
%   \includegraphics[width=0.45\linewidth]{figs/expB/tab_dev.png}
%   \caption{Results of out-of-domain evaluation of the best openSMILE %features. Rows indiciate training attack and feature used, while columns %indicate evaluation performance for all remaining attacks (i.e. out-of-%domain) except diagonal.}
%    \label{fig:enter-label}
%\end{figure*}
\begin{table*}[]
\centering
\caption{Results of out-of-domain evaluation.
% of the best openSMILE features.
Rows indicate
training attack and openSMILE feature used, while columns indicate evaluation attack.
Note that the values on the diagonal originate from identical train and test attacks, and thus represent in-domain evaluation. Note the discrepancy in performance between `train' and `dev' partitions.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|rrrrrrrr|rrrrrrrr}
\hline
  %
  % add here a multi-col for train and dev
  & & \multicolumn{8}{c|}{ASVspoof 5 `train'} & \multicolumn{8}{c|}{ASVspoof 5 `dev'} \\
\hline
  %
 &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} \\
 &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} \\
\multirow{-3}{*}{Attack $\downarrow$} &
  \multirow{-3}{*}{Feature $\downarrow$} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A01}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A02}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A03}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A04}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A05}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A06}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A07}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A08}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A09}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A10}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A11}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A12}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A13}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A14}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A15}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A16}} \\ \hline
 &
  F66 &
  \cellcolor[HTML]{86C280}12.8 &
  \cellcolor[HTML]{86C280}12.7 &
  \cellcolor[HTML]{92C47E}15.7 &
  \cellcolor[HTML]{A9C879}21.7 &
  \cellcolor[HTML]{D0CE70}31.5 &
  \cellcolor[HTML]{B9CA75}25.7 &
  \cellcolor[HTML]{8AC380}13.7 &
  \cellcolor[HTML]{9BC67C}18.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}69.5 &
  \cellcolor[HTML]{E67C73}68.1 &
  \cellcolor[HTML]{E67C73}70.3 &
  \cellcolor[HTML]{E67C73}60.0 &
  \cellcolor[HTML]{E67C73}55.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}76.2 \\ \cline{2-2}
 &
  F19 &
  \cellcolor[HTML]{8AC37F}13.8 &
  \cellcolor[HTML]{87C280}13.0 &
  \cellcolor[HTML]{90C47E}15.3 &
  \cellcolor[HTML]{96C57D}16.8 &
  \cellcolor[HTML]{A0C67B}19.4 &
  \cellcolor[HTML]{97C57D}17.1 &
  \cellcolor[HTML]{9AC57C}17.8 &
  \cellcolor[HTML]{AFC978}23.0 &
  \cellcolor[HTML]{E67C73}61.9 &
  \cellcolor[HTML]{E67C73}62.8 &
  \cellcolor[HTML]{E67C73}55.7 &
  \cellcolor[HTML]{E67C73}78.7 &
  \cellcolor[HTML]{E67C73}54.7 &
  \cellcolor[HTML]{E67C73}54.5 &
  \cellcolor[HTML]{E67C73}65.3 &
  \cellcolor[HTML]{E67C73}66.7 \\ \cline{2-2}
\multirow{-3}{*}{A01} &
  F17 &
  \cellcolor[HTML]{8EC37F}14.7 &
  \cellcolor[HTML]{89C380}13.6 &
  \cellcolor[HTML]{92C47E}15.8 &
  \cellcolor[HTML]{A5C77A}20.5 &
  \cellcolor[HTML]{A3C77A}20.0 &
  \cellcolor[HTML]{A0C67B}19.3 &
  \cellcolor[HTML]{8DC37F}14.6 &
  \cellcolor[HTML]{A3C77A}20.2 &
  \cellcolor[HTML]{E67C73}62.0 &
  \cellcolor[HTML]{E67C73}63.8 &
  \cellcolor[HTML]{E67C73}58.3 &
  \cellcolor[HTML]{E67C73}75.6 &
  \cellcolor[HTML]{E67C73}52.8 &
  \cellcolor[HTML]{E67C73}64.4 &
  \cellcolor[HTML]{E67C73}65.2 &
  \cellcolor[HTML]{E67C73}65.5 \\ \cline{1-2}
 &
  F66 &
  \cellcolor[HTML]{86C280}12.8 &
  \cellcolor[HTML]{86C280}12.7 &
  \cellcolor[HTML]{92C47E}15.7 &
  \cellcolor[HTML]{A9C879}21.7 &
  \cellcolor[HTML]{D0CE70}31.5 &
  \cellcolor[HTML]{B9CA75}25.7 &
  \cellcolor[HTML]{8AC380}13.7 &
  \cellcolor[HTML]{9BC67C}18.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}69.5 &
  \cellcolor[HTML]{E67C73}68.1 &
  \cellcolor[HTML]{E67C73}70.3 &
  \cellcolor[HTML]{E67C73}60.0 &
  \cellcolor[HTML]{E67C73}55.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}76.2 \\ \cline{2-2}
 &
  F19 &
  \cellcolor[HTML]{8AC37F}13.8 &
  \cellcolor[HTML]{87C280}13.0 &
  \cellcolor[HTML]{90C47E}15.3 &
  \cellcolor[HTML]{96C57D}16.8 &
  \cellcolor[HTML]{A0C67B}19.4 &
  \cellcolor[HTML]{97C57D}17.1 &
  \cellcolor[HTML]{9AC57C}17.8 &
  \cellcolor[HTML]{AFC978}23.0 &
  \cellcolor[HTML]{E67C73}61.9 &
  \cellcolor[HTML]{E67C73}62.8 &
  \cellcolor[HTML]{E67C73}55.7 &
  \cellcolor[HTML]{E67C73}78.7 &
  \cellcolor[HTML]{E67C73}54.7 &
  \cellcolor[HTML]{E67C73}54.5 &
  \cellcolor[HTML]{E67C73}65.3 &
  \cellcolor[HTML]{E67C73}66.7 \\ \cline{2-2}
\multirow{-3}{*}{A02} &
  F17 &
  \cellcolor[HTML]{8EC37F}14.7 &
  \cellcolor[HTML]{89C380}13.6 &
  \cellcolor[HTML]{92C47E}15.8 &
  \cellcolor[HTML]{A5C77A}20.5 &
  \cellcolor[HTML]{A3C77A}20.0 &
  \cellcolor[HTML]{A0C67B}19.3 &
  \cellcolor[HTML]{8DC37F}14.6 &
  \cellcolor[HTML]{A3C77A}20.2 &
  \cellcolor[HTML]{E67C73}62.0 &
  \cellcolor[HTML]{E67C73}63.8 &
  \cellcolor[HTML]{E67C73}58.3 &
  \cellcolor[HTML]{E67C73}75.6 &
  \cellcolor[HTML]{E67C73}52.8 &
  \cellcolor[HTML]{E67C73}64.4 &
  \cellcolor[HTML]{E67C73}65.2 &
  \cellcolor[HTML]{E67C73}65.5 \\ \cline{1-2}
 &
  F19 &
  \cellcolor[HTML]{8AC37F}13.8 &
  \cellcolor[HTML]{87C280}13.0 &
  \cellcolor[HTML]{90C47E}15.3 &
  \cellcolor[HTML]{96C57D}16.8 &
  \cellcolor[HTML]{A0C67B}19.4 &
  \cellcolor[HTML]{97C57D}17.1 &
  \cellcolor[HTML]{9AC57C}17.8 &
  \cellcolor[HTML]{AFC978}23.0 &
  \cellcolor[HTML]{E67C73}61.9 &
  \cellcolor[HTML]{E67C73}62.8 &
  \cellcolor[HTML]{E67C73}55.7 &
  \cellcolor[HTML]{E67C73}78.7 &
  \cellcolor[HTML]{E67C73}54.7 &
  \cellcolor[HTML]{E67C73}54.5 &
  \cellcolor[HTML]{E67C73}65.3 &
  \cellcolor[HTML]{E67C73}66.7 \\ \cline{2-2}
 &
  F66 &
  \cellcolor[HTML]{86C280}12.8 &
  \cellcolor[HTML]{86C280}12.7 &
  \cellcolor[HTML]{92C47E}15.7 &
  \cellcolor[HTML]{A9C879}21.7 &
  \cellcolor[HTML]{D0CE70}31.5 &
  \cellcolor[HTML]{B9CA75}25.7 &
  \cellcolor[HTML]{8AC380}13.7 &
  \cellcolor[HTML]{9BC67C}18.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}69.5 &
  \cellcolor[HTML]{E67C73}68.1 &
  \cellcolor[HTML]{E67C73}70.3 &
  \cellcolor[HTML]{E67C73}60.0 &
  \cellcolor[HTML]{E67C73}55.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}76.2 \\ \cline{2-2}
\multirow{-3}{*}{A03} &
  F17 &
  \cellcolor[HTML]{8EC37F}14.7 &
  \cellcolor[HTML]{89C380}13.6 &
  \cellcolor[HTML]{92C47E}15.8 &
  \cellcolor[HTML]{A5C77A}20.5 &
  \cellcolor[HTML]{A3C77A}20.0 &
  \cellcolor[HTML]{A0C67B}19.3 &
  \cellcolor[HTML]{8DC37F}14.6 &
  \cellcolor[HTML]{A3C77A}20.2 &
  \cellcolor[HTML]{E67C73}62.0 &
  \cellcolor[HTML]{E67C73}63.8 &
  \cellcolor[HTML]{E67C73}58.3 &
  \cellcolor[HTML]{E67C73}75.6 &
  \cellcolor[HTML]{E67C73}52.8 &
  \cellcolor[HTML]{E67C73}64.4 &
  \cellcolor[HTML]{E67C73}65.2 &
  \cellcolor[HTML]{E67C73}65.5 \\ \cline{1-2}
 &
  F19 &
  \cellcolor[HTML]{8AC37F}13.8 &
  \cellcolor[HTML]{87C280}13.0 &
  \cellcolor[HTML]{90C47E}15.3 &
  \cellcolor[HTML]{96C57D}16.8 &
  \cellcolor[HTML]{A0C67B}19.4 &
  \cellcolor[HTML]{97C57D}17.1 &
  \cellcolor[HTML]{9AC57C}17.8 &
  \cellcolor[HTML]{AFC978}23.0 &
  \cellcolor[HTML]{E67C73}61.9 &
  \cellcolor[HTML]{E67C73}62.8 &
  \cellcolor[HTML]{E67C73}55.7 &
  \cellcolor[HTML]{E67C73}78.7 &
  \cellcolor[HTML]{E67C73}54.7 &
  \cellcolor[HTML]{E67C73}54.5 &
  \cellcolor[HTML]{E67C73}65.3 &
  \cellcolor[HTML]{E67C73}66.7 \\ \cline{2-2}
 &
  F21 &
  \cellcolor[HTML]{AAC879}21.9 &
  \cellcolor[HTML]{A9C879}21.6 &
  \cellcolor[HTML]{B6CA76}24.8 &
  \cellcolor[HTML]{98C57C}17.3 &
  \cellcolor[HTML]{99C57C}17.5 &
  \cellcolor[HTML]{96C57D}16.8 &
  \cellcolor[HTML]{9DC67B}18.7 &
  \cellcolor[HTML]{F6B66A}45.7 &
  \cellcolor[HTML]{9BC67C}18.1 &
  \cellcolor[HTML]{99C57C}17.5 &
  \cellcolor[HTML]{F2D369}40.0 &
  \cellcolor[HTML]{FED066}43.7 &
  \cellcolor[HTML]{D9D06E}33.8 &
  \cellcolor[HTML]{C5CC73}28.6 &
  \cellcolor[HTML]{E4D16C}36.5 &
  \cellcolor[HTML]{F8D468}41.5 \\ \cline{2-2}
\multirow{-3}{*}{A04} &
  F81 &
  \cellcolor[HTML]{CCCD71}30.5 &
  \cellcolor[HTML]{D2CE70}31.8 &
  \cellcolor[HTML]{D7CF6F}33.2 &
  \cellcolor[HTML]{A3C77A}20.1 &
  \cellcolor[HTML]{B4C977}24.3 &
  \cellcolor[HTML]{B6CA76}24.8 &
  \cellcolor[HTML]{D2CE70}32.0 &
  \cellcolor[HTML]{E67C73}59.0 &
  \cellcolor[HTML]{ADC878}22.5 &
  \cellcolor[HTML]{A7C779}21.2 &
  \cellcolor[HTML]{E67C73}52.8 &
  \cellcolor[HTML]{C3CC73}28.2 &
  \cellcolor[HTML]{FED567}43.0 &
  \cellcolor[HTML]{D2CE70}31.8 &
  \cellcolor[HTML]{F7D468}41.4 &
  \cellcolor[HTML]{ECD36A}38.6 \\ \cline{1-2}
 &
  F21 &
  \cellcolor[HTML]{AAC879}21.9 &
  \cellcolor[HTML]{A9C879}21.6 &
  \cellcolor[HTML]{B6CA76}24.8 &
  \cellcolor[HTML]{98C57C}17.3 &
  \cellcolor[HTML]{99C57C}17.5 &
  \cellcolor[HTML]{96C57D}16.8 &
  \cellcolor[HTML]{9DC67B}18.7 &
  \cellcolor[HTML]{F6B66A}45.7 &
  \cellcolor[HTML]{9BC67C}18.1 &
  \cellcolor[HTML]{99C57C}17.5 &
  \cellcolor[HTML]{F2D369}40.0 &
  \cellcolor[HTML]{FED066}43.7 &
  \cellcolor[HTML]{D9D06E}33.8 &
  \cellcolor[HTML]{C5CC73}28.6 &
  \cellcolor[HTML]{E4D16C}36.5 &
  \cellcolor[HTML]{F8D468}41.5 \\ \cline{2-2}
 &
  F19 &
  \cellcolor[HTML]{8AC37F}13.8 &
  \cellcolor[HTML]{87C280}13.0 &
  \cellcolor[HTML]{90C47E}15.3 &
  \cellcolor[HTML]{96C57D}16.8 &
  \cellcolor[HTML]{A0C67B}19.4 &
  \cellcolor[HTML]{97C57D}17.1 &
  \cellcolor[HTML]{9AC57C}17.8 &
  \cellcolor[HTML]{AFC978}23.0 &
  \cellcolor[HTML]{E67C73}61.9 &
  \cellcolor[HTML]{E67C73}62.8 &
  \cellcolor[HTML]{E67C73}55.7 &
  \cellcolor[HTML]{E67C73}78.7 &
  \cellcolor[HTML]{E67C73}54.7 &
  \cellcolor[HTML]{E67C73}54.5 &
  \cellcolor[HTML]{E67C73}65.3 &
  \cellcolor[HTML]{E67C73}66.7 \\ \cline{2-2}
\multirow{-3}{*}{A05} &
  F17 &
  \cellcolor[HTML]{8EC37F}14.7 &
  \cellcolor[HTML]{89C380}13.6 &
  \cellcolor[HTML]{92C47E}15.8 &
  \cellcolor[HTML]{A5C77A}20.5 &
  \cellcolor[HTML]{A3C77A}20.0 &
  \cellcolor[HTML]{A0C67B}19.3 &
  \cellcolor[HTML]{8DC37F}14.6 &
  \cellcolor[HTML]{A3C77A}20.2 &
  \cellcolor[HTML]{E67C73}62.0 &
  \cellcolor[HTML]{E67C73}63.8 &
  \cellcolor[HTML]{E67C73}58.3 &
  \cellcolor[HTML]{E67C73}75.6 &
  \cellcolor[HTML]{E67C73}52.8 &
  \cellcolor[HTML]{E67C73}64.4 &
  \cellcolor[HTML]{E67C73}65.2 &
  \cellcolor[HTML]{E67C73}65.5 \\ \cline{1-2}
 &
  F21 &
  \cellcolor[HTML]{AAC879}21.9 &
  \cellcolor[HTML]{A9C879}21.6 &
  \cellcolor[HTML]{B6CA76}24.8 &
  \cellcolor[HTML]{98C57C}17.3 &
  \cellcolor[HTML]{99C57C}17.5 &
  \cellcolor[HTML]{96C57D}16.8 &
  \cellcolor[HTML]{9DC67B}18.7 &
  \cellcolor[HTML]{F6B66A}45.7 &
  \cellcolor[HTML]{9BC67C}18.1 &
  \cellcolor[HTML]{99C57C}17.5 &
  \cellcolor[HTML]{F2D369}40.0 &
  \cellcolor[HTML]{FED066}43.7 &
  \cellcolor[HTML]{D9D06E}33.8 &
  \cellcolor[HTML]{C5CC73}28.6 &
  \cellcolor[HTML]{E4D16C}36.5 &
  \cellcolor[HTML]{F8D468}41.5 \\ \cline{2-2}
 &
  F19 &
  \cellcolor[HTML]{8AC37F}13.8 &
  \cellcolor[HTML]{87C280}13.0 &
  \cellcolor[HTML]{90C47E}15.3 &
  \cellcolor[HTML]{96C57D}16.8 &
  \cellcolor[HTML]{A0C67B}19.4 &
  \cellcolor[HTML]{97C57D}17.1 &
  \cellcolor[HTML]{9AC57C}17.8 &
  \cellcolor[HTML]{AFC978}23.0 &
  \cellcolor[HTML]{E67C73}61.9 &
  \cellcolor[HTML]{E67C73}62.8 &
  \cellcolor[HTML]{E67C73}55.7 &
  \cellcolor[HTML]{E67C73}78.7 &
  \cellcolor[HTML]{E67C73}54.7 &
  \cellcolor[HTML]{E67C73}54.5 &
  \cellcolor[HTML]{E67C73}65.3 &
  \cellcolor[HTML]{E67C73}66.7 \\ \cline{2-2}
\multirow{-3}{*}{A06} &
  F17 &
  \cellcolor[HTML]{8EC37F}14.7 &
  \cellcolor[HTML]{89C380}13.6 &
  \cellcolor[HTML]{92C47E}15.8 &
  \cellcolor[HTML]{A5C77A}20.5 &
  \cellcolor[HTML]{A3C77A}20.0 &
  \cellcolor[HTML]{A0C67B}19.3 &
  \cellcolor[HTML]{8DC37F}14.6 &
  \cellcolor[HTML]{A3C77A}20.2 &
  \cellcolor[HTML]{E67C73}62.0 &
  \cellcolor[HTML]{E67C73}63.8 &
  \cellcolor[HTML]{E67C73}58.3 &
  \cellcolor[HTML]{E67C73}75.6 &
  \cellcolor[HTML]{E67C73}52.8 &
  \cellcolor[HTML]{E67C73}64.4 &
  \cellcolor[HTML]{E67C73}65.2 &
  \cellcolor[HTML]{E67C73}65.5 \\ \cline{1-2}
 &
  F66 &
  \cellcolor[HTML]{86C280}12.8 &
  \cellcolor[HTML]{86C280}12.7 &
  \cellcolor[HTML]{92C47E}15.7 &
  \cellcolor[HTML]{A9C879}21.7 &
  \cellcolor[HTML]{D0CE70}31.5 &
  \cellcolor[HTML]{B9CA75}25.7 &
  \cellcolor[HTML]{8AC380}13.7 &
  \cellcolor[HTML]{9BC67C}18.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}69.5 &
  \cellcolor[HTML]{E67C73}68.1 &
  \cellcolor[HTML]{E67C73}70.3 &
  \cellcolor[HTML]{E67C73}60.0 &
  \cellcolor[HTML]{E67C73}55.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}76.2 \\ \cline{2-2}
 &
  F1 &
  \cellcolor[HTML]{D6CF6F}32.9 &
  \cellcolor[HTML]{CECE71}31.0 &
  \cellcolor[HTML]{C8CD72}29.5 &
  \cellcolor[HTML]{E6D26C}37.0 &
  \cellcolor[HTML]{C6CC73}29.0 &
  \cellcolor[HTML]{D5CF6F}32.7 &
  \cellcolor[HTML]{8CC37F}14.2 &
  \cellcolor[HTML]{DCD06E}34.4 &
  \cellcolor[HTML]{DDD06E}34.8 &
  \cellcolor[HTML]{DCD06E}34.3 &
  \cellcolor[HTML]{E67C73}50.7 &
  \cellcolor[HTML]{E88272}49.6 &
  \cellcolor[HTML]{C6CC73}28.8 &
  \cellcolor[HTML]{A4C77A}20.3 &
  \cellcolor[HTML]{DAD06E}33.8 &
  \cellcolor[HTML]{E0D16D}35.6 \\ \cline{2-2}
\multirow{-3}{*}{A07} &
  F17 &
  \cellcolor[HTML]{8EC37F}14.7 &
  \cellcolor[HTML]{89C380}13.6 &
  \cellcolor[HTML]{92C47E}15.8 &
  \cellcolor[HTML]{A5C77A}20.5 &
  \cellcolor[HTML]{A3C77A}20.0 &
  \cellcolor[HTML]{A0C67B}19.3 &
  \cellcolor[HTML]{8DC37F}14.6 &
  \cellcolor[HTML]{A3C77A}20.2 &
  \cellcolor[HTML]{E67C73}62.0 &
  \cellcolor[HTML]{E67C73}63.8 &
  \cellcolor[HTML]{E67C73}58.3 &
  \cellcolor[HTML]{E67C73}75.6 &
  \cellcolor[HTML]{E67C73}52.8 &
  \cellcolor[HTML]{E67C73}64.4 &
  \cellcolor[HTML]{E67C73}65.2 &
  \cellcolor[HTML]{E67C73}65.5 \\ \cline{1-2}
 &
  F20 &
  \cellcolor[HTML]{98C57D}17.2 &
  \cellcolor[HTML]{98C57D}17.2 &
  \cellcolor[HTML]{9EC67B}18.8 &
  \cellcolor[HTML]{C3CC73}28.2 &
  \cellcolor[HTML]{E2D16D}36.1 &
  \cellcolor[HTML]{CECE71}30.9 &
  \cellcolor[HTML]{A2C77A}19.9 &
  \cellcolor[HTML]{9AC57C}17.7 &
  \cellcolor[HTML]{E67C73}77.7 &
  \cellcolor[HTML]{E67C73}79.0 &
  \cellcolor[HTML]{E67C73}69.2 &
  \cellcolor[HTML]{E67C73}70.9 &
  \cellcolor[HTML]{E67C73}60.8 &
  \cellcolor[HTML]{E67C73}89.0 &
  \cellcolor[HTML]{E67C73}67.5 &
  \cellcolor[HTML]{E67C73}72.7 \\ \cline{2-2}
 &
  F66 &
  \cellcolor[HTML]{86C280}12.8 &
  \cellcolor[HTML]{86C280}12.7 &
  \cellcolor[HTML]{92C47E}15.7 &
  \cellcolor[HTML]{A9C879}21.7 &
  \cellcolor[HTML]{D0CE70}31.5 &
  \cellcolor[HTML]{B9CA75}25.7 &
  \cellcolor[HTML]{8AC380}13.7 &
  \cellcolor[HTML]{9BC67C}18.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}69.5 &
  \cellcolor[HTML]{E67C73}68.1 &
  \cellcolor[HTML]{E67C73}70.3 &
  \cellcolor[HTML]{E67C73}60.0 &
  \cellcolor[HTML]{E67C73}55.2 &
  \cellcolor[HTML]{E67C73}68.7 &
  \cellcolor[HTML]{E67C73}76.2 \\ \cline{2-2}
\multirow{-3}{*}{A08} &
  F17 &
  \cellcolor[HTML]{8EC37F}14.7 &
  \cellcolor[HTML]{89C380}13.6 &
  \cellcolor[HTML]{92C47E}15.8 &
  \cellcolor[HTML]{A5C77A}20.5 &
  \cellcolor[HTML]{A3C77A}20.0 &
  \cellcolor[HTML]{A0C67B}19.3 &
  \cellcolor[HTML]{8DC37F}14.6 &
  \cellcolor[HTML]{A3C77A}20.2 &
  \cellcolor[HTML]{E67C73}62.0 &
  \cellcolor[HTML]{E67C73}63.8 &
  \cellcolor[HTML]{E67C73}58.3 &
  \cellcolor[HTML]{E67C73}75.6 &
  \cellcolor[HTML]{E67C73}52.8 &
  \cellcolor[HTML]{E67C73}64.4 &
  \cellcolor[HTML]{E67C73}65.2 &
  \cellcolor[HTML]{E67C73}65.5 \\ \hline
 &
  F86 &
  \cellcolor[HTML]{C7CD72}26.3 &
  \cellcolor[HTML]{B5CA76}22.3 &
  \cellcolor[HTML]{BDCB75}23.9 &
  \cellcolor[HTML]{D0CE71}28.2 &
  \cellcolor[HTML]{BACA75}23.3 &
  \cellcolor[HTML]{BECB74}24.2 &
  \cellcolor[HTML]{AEC978}20.6 &
  \cellcolor[HTML]{E77E72}49.8 &
  \cellcolor[HTML]{77C084} 8.0 &
  \cellcolor[HTML]{74BF84} 7.3 &
  \cellcolor[HTML]{E67C73}61.5 &
  \cellcolor[HTML]{FBD567}38.0 &
  \cellcolor[HTML]{E98571}49.0 &
  \cellcolor[HTML]{E67C73}65.0 &
  \cellcolor[HTML]{F1A16D}45.5 &
  \cellcolor[HTML]{F5B26B}43.3 \\ \cline{2-2}
 &
  F85 &
  \cellcolor[HTML]{FCD567}38.3 &
  \cellcolor[HTML]{FDCD67}40.0 &
  \cellcolor[HTML]{F3D469}36.2 &
  \cellcolor[HTML]{FCD567}38.3 &
  \cellcolor[HTML]{F3D469}36.2 &
  \cellcolor[HTML]{F9D568}37.5 &
  \cellcolor[HTML]{D6CF6F}29.5 &
  \cellcolor[HTML]{E67C73}53.9 &
  \cellcolor[HTML]{86C280}11.5 &
  \cellcolor[HTML]{82C281}10.7 &
  \cellcolor[HTML]{E67C73}63.2 &
  \cellcolor[HTML]{ECD36A}34.7 &
  \cellcolor[HTML]{E67C73}68.0 &
  \cellcolor[HTML]{E67C73}97.0 &
  \cellcolor[HTML]{EE976F}46.8 &
  \cellcolor[HTML]{F2A56D}45.0 \\ \cline{2-2}
\multirow{-3}{*}{A09} &
  F12 &
  \cellcolor[HTML]{F1A16D}45.5 &
  \cellcolor[HTML]{F4AB6C}44.2 &
  \cellcolor[HTML]{EE966F}46.8 &
  \cellcolor[HTML]{F8BC69}42.1 &
  \cellcolor[HTML]{FED266}39.3 &
  \cellcolor[HTML]{FFD366}39.2 &
  \cellcolor[HTML]{FED567}38.7 &
  \cellcolor[HTML]{E67C73}65.0 &
  \cellcolor[HTML]{8BC37F}12.7 &
  \cellcolor[HTML]{89C380}12.2 &
  \cellcolor[HTML]{EB8D70}48.0 &
  \cellcolor[HTML]{FED266}39.3 &
  \cellcolor[HTML]{D4CF70}29.2 &
  \cellcolor[HTML]{A3C77A}18.2 &
  \cellcolor[HTML]{EFD36A}35.3 &
  \cellcolor[HTML]{F6D468}36.9 \\ \cline{1-2}
 &
  F86 &
  \cellcolor[HTML]{C7CD72}26.3 &
  \cellcolor[HTML]{B5CA76}22.3 &
  \cellcolor[HTML]{BDCB75}23.9 &
  \cellcolor[HTML]{D0CE71}28.2 &
  \cellcolor[HTML]{BACA75}23.3 &
  \cellcolor[HTML]{BECB74}24.2 &
  \cellcolor[HTML]{AEC978}20.6 &
  \cellcolor[HTML]{E77E72}49.8 &
  \cellcolor[HTML]{77C084} 8.0 &
  \cellcolor[HTML]{74BF84} 7.3 &
  \cellcolor[HTML]{E67C73}61.5 &
  \cellcolor[HTML]{FBD567}38.0 &
  \cellcolor[HTML]{E98571}49.0 &
  \cellcolor[HTML]{E67C73}65.0 &
  \cellcolor[HTML]{F1A16D}45.5 &
  \cellcolor[HTML]{F2A56D}45.0 \\ \cline{2-2}
 &
  F85 &
  \cellcolor[HTML]{FCD567}38.3 &
  \cellcolor[HTML]{FDCD67}40.0 &
  \cellcolor[HTML]{F3D469}36.2 &
  \cellcolor[HTML]{FCD567}38.3 &
  \cellcolor[HTML]{F3D469}36.2 &
  \cellcolor[HTML]{F9D568}37.5 &
  \cellcolor[HTML]{D6CF6F}29.5 &
  \cellcolor[HTML]{E67C73}53.9 &
  \cellcolor[HTML]{86C280}11.5 &
  \cellcolor[HTML]{82C281}10.7 &
  \cellcolor[HTML]{E67C73}63.2 &
  \cellcolor[HTML]{ECD36A}34.7 &
  \cellcolor[HTML]{E67C73}68.0 &
  \cellcolor[HTML]{E67C73}97.0 &
  \cellcolor[HTML]{EE976F}46.8 &
  \cellcolor[HTML]{F5B26B}43.3 \\ \cline{2-2}
\multirow{-3}{*}{A10} &
  F12 &
  \cellcolor[HTML]{F1A16D}45.5 &
  \cellcolor[HTML]{F4AB6C}44.2 &
  \cellcolor[HTML]{EE966F}46.8 &
  \cellcolor[HTML]{F8BC69}42.1 &
  \cellcolor[HTML]{FED266}39.3 &
  \cellcolor[HTML]{FFD366}39.2 &
  \cellcolor[HTML]{FED567}38.7 &
  \cellcolor[HTML]{E67C73}65.0 &
  \cellcolor[HTML]{8BC37F}12.7 &
  \cellcolor[HTML]{89C380}12.2 &
  \cellcolor[HTML]{EB8D70}48.0 &
  \cellcolor[HTML]{FED266}39.3 &
  \cellcolor[HTML]{D4CF70}29.2 &
  \cellcolor[HTML]{A3C77A}18.2 &
  \cellcolor[HTML]{EFD36A}35.3 &
  \cellcolor[HTML]{F6D468}36.9 \\ \cline{1-2}
 &
  F58 &
  \cellcolor[HTML]{EA8871}48.6 &
  \cellcolor[HTML]{E67C73}50.3 &
  \cellcolor[HTML]{E88372}49.3 &
  \cellcolor[HTML]{E88272}49.3 &
  \cellcolor[HTML]{F3AA6C}44.3 &
  \cellcolor[HTML]{F7B76A}42.7 &
  \cellcolor[HTML]{FAC169}41.4 &
  \cellcolor[HTML]{EB8D70}48.0 &
  \cellcolor[HTML]{F4D469}36.5 &
  \cellcolor[HTML]{FCD567}38.2 &
  \cellcolor[HTML]{97C57D}15.3 &
  \cellcolor[HTML]{E67C73}51.3 &
  \cellcolor[HTML]{E67C73}50.8 &
  \cellcolor[HTML]{E67C73}54.8 &
  \cellcolor[HTML]{FFD566}38.9 &
  \cellcolor[HTML]{E77F72}49.7 \\ \cline{2-2}
 &
  F60 &
  \cellcolor[HTML]{EF9B6E}46.2 &
  \cellcolor[HTML]{EB8D70}48.0 &
  \cellcolor[HTML]{EF9D6E}46.0 &
  \cellcolor[HTML]{E98671}48.8 &
  \cellcolor[HTML]{F5B16B}43.5 &
  \cellcolor[HTML]{FBC768}40.7 &
  \cellcolor[HTML]{FCCB67}40.3 &
  \cellcolor[HTML]{EF9B6E}46.3 &
  \cellcolor[HTML]{F0D36A}35.6 &
  \cellcolor[HTML]{FAD567}37.8 &
  \cellcolor[HTML]{97C57D}15.3 &
  \cellcolor[HTML]{E67C73}52.6 &
  \cellcolor[HTML]{E98571}49.0 &
  \cellcolor[HTML]{E67C73}58.7 &
  \cellcolor[HTML]{F8D468}37.3 &
  \cellcolor[HTML]{FBC768}40.7 \\ \cline{2-2}
\multirow{-3}{*}{A11} &
  F59 &
  \cellcolor[HTML]{FDCE67}39.8 &
  \cellcolor[HTML]{F8D468}37.3 &
  \cellcolor[HTML]{FCC967}40.5 &
  \cellcolor[HTML]{EA8A71}48.3 &
  \cellcolor[HTML]{FFD366}39.2 &
  \cellcolor[HTML]{F8D468}37.3 &
  \cellcolor[HTML]{E1D16D}32.2 &
  \cellcolor[HTML]{F9BF69}41.7 &
  \cellcolor[HTML]{FED567}38.6 &
  \cellcolor[HTML]{FAC169}41.4 &
  \cellcolor[HTML]{A1C77A}17.7 &
  \cellcolor[HTML]{E67C73}50.5 &
  \cellcolor[HTML]{D3CE70}28.8 &
  \cellcolor[HTML]{87C280}11.8 &
  \cellcolor[HTML]{F4D469}36.5 &
  \cellcolor[HTML]{F9C169}41.5 \\ \cline{1-2}
 &
  F82 &
  \cellcolor[HTML]{EAD26B}34.1 &
  \cellcolor[HTML]{E7D26B}33.6 &
  \cellcolor[HTML]{F3D469}36.2 &
  \cellcolor[HTML]{D5CF6F}29.3 &
  \cellcolor[HTML]{D6CF6F}29.6 &
  \cellcolor[HTML]{D2CE70}28.7 &
  \cellcolor[HTML]{EC9070}47.6 &
  \cellcolor[HTML]{E67C73}60.2 &
  \cellcolor[HTML]{F5D469}36.6 &
  \cellcolor[HTML]{EBD26B}34.3 &
  \cellcolor[HTML]{E67C73}64.5 &
  \cellcolor[HTML]{A3C77A}18.2 &
  \cellcolor[HTML]{E67C73}66.1 &
  \cellcolor[HTML]{E67C73}94.0 &
  \cellcolor[HTML]{F6B36B}43.2 &
  \cellcolor[HTML]{E67C73}51.3 \\ \cline{2-2}
 &
  F19 &
  \cellcolor[HTML]{E67C73}86.2 &
  \cellcolor[HTML]{E67C73}87.0 &
  \cellcolor[HTML]{E67C73}84.7 &
  \cellcolor[HTML]{E67C73}83.3 &
  \cellcolor[HTML]{E67C73}80.6 &
  \cellcolor[HTML]{E67C73}82.9 &
  \cellcolor[HTML]{E67C73}82.2 &
  \cellcolor[HTML]{E67C73}77.0 &
  \cellcolor[HTML]{FBD567}38.1 &
  \cellcolor[HTML]{F8D468}37.3 &
  \cellcolor[HTML]{F3AA6C}44.3 &
  \cellcolor[HTML]{B1C977}21.3 &
  \cellcolor[HTML]{F1A26D}45.3 &
  \cellcolor[HTML]{F1A16D}45.5 &
  \cellcolor[HTML]{EDD36A}34.8 &
  \cellcolor[HTML]{E6D26C}33.3 \\ \cline{2-2}
\multirow{-3}{*}{A12} &
  F83 &
  \cellcolor[HTML]{FBC768}40.7 &
  \cellcolor[HTML]{FFD366}39.2 &
  \cellcolor[HTML]{F2A56D}45.0 &
  \cellcolor[HTML]{E5D16C}33.1 &
  \cellcolor[HTML]{F7D468}37.2 &
  \cellcolor[HTML]{EED36A}35.0 &
  \cellcolor[HTML]{E67C73}61.4 &
  \cellcolor[HTML]{E67C73}56.5 &
  \cellcolor[HTML]{E67C73}61.3 &
  \cellcolor[HTML]{E67C73}60.7 &
  \cellcolor[HTML]{EA8971}48.5 &
  \cellcolor[HTML]{B8CA76}22.8 &
  \cellcolor[HTML]{EED36A}35.2 &
  \cellcolor[HTML]{5BBB89} 1.8 &
  \cellcolor[HTML]{F6B36B}43.2 &
  \cellcolor[HTML]{E67C73}55.1 \\ \cline{1-2}
 &
  F67 &
  \cellcolor[HTML]{E1D16D}32.0 &
  \cellcolor[HTML]{DAD06E}30.6 &
  \cellcolor[HTML]{EAD26B}34.1 &
  \cellcolor[HTML]{C2CC74}25.0 &
  \cellcolor[HTML]{C0CB74}24.6 &
  \cellcolor[HTML]{C3CC73}25.3 &
  \cellcolor[HTML]{C1CC74}24.8 &
  \cellcolor[HTML]{FFD566}39.0 &
  \cellcolor[HTML]{FBC768}40.7 &
  \cellcolor[HTML]{FECF67}39.7 &
  \cellcolor[HTML]{E6D26C}33.2 &
  \cellcolor[HTML]{E88172}49.5 &
  \cellcolor[HTML]{B5CA76}22.1 &
  \cellcolor[HTML]{95C57D}15.0 &
  \cellcolor[HTML]{FBD567}38.1 &
  \cellcolor[HTML]{F1D369}35.8 \\ \cline{2-2}
 &
  F39 &
  \cellcolor[HTML]{F3D469}36.1 &
  \cellcolor[HTML]{E6D26C}33.3 &
  \cellcolor[HTML]{F8D468}37.3 &
  \cellcolor[HTML]{F7B96A}42.5 &
  \cellcolor[HTML]{E8D26B}33.7 &
  \cellcolor[HTML]{E7D26C}33.4 &
  \cellcolor[HTML]{C5CC73}25.8 &
  \cellcolor[HTML]{FBD567}37.9 &
  \cellcolor[HTML]{FDD567}38.4 &
  \cellcolor[HTML]{FCC967}40.5 &
  \cellcolor[HTML]{D2CE70}28.7 &
  \cellcolor[HTML]{E88272}49.3 &
  \cellcolor[HTML]{B8CA76}22.8 &
  \cellcolor[HTML]{ACC878}20.1 &
  \cellcolor[HTML]{F6D468}36.8 &
  \cellcolor[HTML]{E5D16C}33.0 \\ \cline{2-2}
\multirow{-3}{*}{A13} &
  F49 &
  \cellcolor[HTML]{F3AB6C}44.3 &
  \cellcolor[HTML]{F8BA6A}42.3 &
  \cellcolor[HTML]{F09E6E}45.8 &
  \cellcolor[HTML]{E67C73}51.3 &
  \cellcolor[HTML]{EB8E70}47.8 &
  \cellcolor[HTML]{E98671}48.8 &
  \cellcolor[HTML]{F9BF69}41.8 &
  \cellcolor[HTML]{E98671}48.8 &
  \cellcolor[HTML]{EC9170}47.5 &
  \cellcolor[HTML]{E88272}49.3 &
  \cellcolor[HTML]{FBC768}40.8 &
  \cellcolor[HTML]{EC926F}47.3 &
  \cellcolor[HTML]{C2CC74}25.0 &
  \cellcolor[HTML]{B7CA76}22.6 &
  \cellcolor[HTML]{FAC268}41.3 &
  \cellcolor[HTML]{FAC268}41.3 \\ \cline{1-2}
 &
  F45 &
  \cellcolor[HTML]{E67C73}52.8 &
  \cellcolor[HTML]{E67C73}53.3 &
  \cellcolor[HTML]{E67C73}56.9 &
  \cellcolor[HTML]{EF9C6E}46.7 &
  \cellcolor[HTML]{E67C73}50.4 &
  \cellcolor[HTML]{EC8F70}48.1 &
  \cellcolor[HTML]{E67C73}71.2 &
  \cellcolor[HTML]{E67C73}55.6 &
  \cellcolor[HTML]{E67C73}80.9 &
  \cellcolor[HTML]{E67C73}80.8 &
  \cellcolor[HTML]{FCD567}39.9 &
  \cellcolor[HTML]{FCCA67}41.8 &
  \cellcolor[HTML]{DBD06E}32.1 &
  \cellcolor[HTML]{57BB8A} 0.8 &
  \cellcolor[HTML]{F2A66C}45.6 &
  \cellcolor[HTML]{E67C73}55.0 \\ \cline{2-2}
 &
  F51 &
  \cellcolor[HTML]{E67C73}51.0 &
  \cellcolor[HTML]{E67C73}51.0 &
  \cellcolor[HTML]{E67C73}54.3 &
  \cellcolor[HTML]{F4AD6B}44.8 &
  \cellcolor[HTML]{F3AA6C}45.2 &
  \cellcolor[HTML]{FBC668}42.3 &
  \cellcolor[HTML]{E67C73}65.0 &
  \cellcolor[HTML]{E67C73}53.2 &
  \cellcolor[HTML]{E67C73}73.8 &
  \cellcolor[HTML]{E67C73}73.8 &
  \cellcolor[HTML]{E5D16C}34.3 &
  \cellcolor[HTML]{F9BF69}43.0 &
  \cellcolor[HTML]{CFCE71}29.3 &
  \cellcolor[HTML]{57BB8A} 0.8 &
  \cellcolor[HTML]{FBC868}42.0 &
  \cellcolor[HTML]{E67C73}56.0 \\ \cline{2-2}
\multirow{-3}{*}{A14} &
  F57 &
  \cellcolor[HTML]{E88172}49.5 &
  \cellcolor[HTML]{EB8E70}48.2 &
  \cellcolor[HTML]{E67C73}52.2 &
  \cellcolor[HTML]{F7B76A}43.8 &
  \cellcolor[HTML]{F8BA6A}43.5 &
  \cellcolor[HTML]{FED567}40.4 &
  \cellcolor[HTML]{E67C73}62.5 &
  \cellcolor[HTML]{E67C73}51.3 &
  \cellcolor[HTML]{E67C73}70.0 &
  \cellcolor[HTML]{E67C73}71.0 &
  \cellcolor[HTML]{DCD06E}32.3 &
  \cellcolor[HTML]{FBC568}42.3 &
  \cellcolor[HTML]{C1CC74}25.8 &
  \cellcolor[HTML]{57BB8A} 0.8 &
  \cellcolor[HTML]{F8D568}39.0 &
  \cellcolor[HTML]{E67C73}51.7 \\ \cline{1-2}
 &
  F78 &
  \cellcolor[HTML]{E67C73}56.2 &
  \cellcolor[HTML]{E67C73}59.7 &
  \cellcolor[HTML]{E67C73}57.7 &
  \cellcolor[HTML]{E67C73}55.7 &
  \cellcolor[HTML]{E67C73}52.2 &
  \cellcolor[HTML]{E67C73}53.2 &
  \cellcolor[HTML]{E67C73}57.8 &
  \cellcolor[HTML]{EA8A71}49.0 &
  \cellcolor[HTML]{FFD666}43.2 &
  \cellcolor[HTML]{FAC368}44.7 &
  \cellcolor[HTML]{F7D468}41.2 &
  \cellcolor[HTML]{E67C73}51.8 &
  \cellcolor[HTML]{E67C73}62.7 &
  \cellcolor[HTML]{E67C73}58.5 &
  \cellcolor[HTML]{A5C77A}20.7 &
  \cellcolor[HTML]{F8BA6A}45.3 \\ \cline{2-2}
 &
  F77 &
  \cellcolor[HTML]{E88272}49.6 &
  \cellcolor[HTML]{E78072}49.8 &
  \cellcolor[HTML]{E67C73}50.3 &
  \cellcolor[HTML]{EB8C70}48.8 &
  \cellcolor[HTML]{EE976F}48.0 &
  \cellcolor[HTML]{EF9C6E}47.6 &
  \cellcolor[HTML]{E67C73}55.3 &
  \cellcolor[HTML]{F8BC69}45.2 &
  \cellcolor[HTML]{ED956F}48.2 &
  \cellcolor[HTML]{EA8B70}48.9 &
  \cellcolor[HTML]{ADC878}22.6 &
  \cellcolor[HTML]{F5B16B}46.0 &
  \cellcolor[HTML]{E67C73}58.3 &
  \cellcolor[HTML]{D0CE71}31.3 &
  \cellcolor[HTML]{B9CA75}25.7 &
  \cellcolor[HTML]{FDCE67}43.8 \\ \cline{2-2}
\multirow{-3}{*}{A15} &
  F76 &
  \cellcolor[HTML]{E77F72}49.8 &
  \cellcolor[HTML]{E67C73}50.3 &
  \cellcolor[HTML]{E67C73}51.7 &
  \cellcolor[HTML]{E67C73}51.0 &
  \cellcolor[HTML]{EC9070}48.5 &
  \cellcolor[HTML]{EB8C70}48.8 &
  \cellcolor[HTML]{E67C73}57.3 &
  \cellcolor[HTML]{F5AF6B}46.2 &
  \cellcolor[HTML]{F3A86C}46.7 &
  \cellcolor[HTML]{F0A06D}47.3 &
  \cellcolor[HTML]{A9C879}21.7 &
  \cellcolor[HTML]{F8BD69}45.1 &
  \cellcolor[HTML]{E67C73}57.2 &
  \cellcolor[HTML]{D2CE70}32.0 &
  \cellcolor[HTML]{BECB74}26.8 &
  \cellcolor[HTML]{E67C73}54.9 \\ \cline{1-2}
 &
  F66 &
  \cellcolor[HTML]{E67C73}87.2 &
  \cellcolor[HTML]{E67C73}87.3 &
  \cellcolor[HTML]{E67C73}84.3 &
  \cellcolor[HTML]{E67C73}78.3 &
  \cellcolor[HTML]{E67C73}68.5 &
  \cellcolor[HTML]{E67C73}74.3 &
  \cellcolor[HTML]{E67C73}86.3 &
  \cellcolor[HTML]{E67C73}81.8 &
  \cellcolor[HTML]{DED06E}31.3 &
  \cellcolor[HTML]{DAD06E}30.5 &
  \cellcolor[HTML]{E0D16D}31.9 &
  \cellcolor[HTML]{D6CF6F}29.7 &
  \cellcolor[HTML]{FDCD67}40.0 &
  \cellcolor[HTML]{F2A66D}44.8 &
  \cellcolor[HTML]{DED06E}31.3 &
  \cellcolor[HTML]{BCCB75}23.8 \\ \cline{2-2}
 &
  F18 &
  \cellcolor[HTML]{E67C73}81.0 &
  \cellcolor[HTML]{E67C73}82.2 &
  \cellcolor[HTML]{E67C73}79.2 &
  \cellcolor[HTML]{E67C73}73.7 &
  \cellcolor[HTML]{E67C73}69.2 &
  \cellcolor[HTML]{E67C73}73.8 &
  \cellcolor[HTML]{E67C73}77.1 &
  \cellcolor[HTML]{E67C73}76.5 &
  \cellcolor[HTML]{DDD06E}31.2 &
  \cellcolor[HTML]{D5CF6F}29.5 &
  \cellcolor[HTML]{F8BA6A}42.3 &
  \cellcolor[HTML]{BFCB74}24.3 &
  \cellcolor[HTML]{EF9B6E}46.3 &
  \cellcolor[HTML]{FAD567}37.8 &
  \cellcolor[HTML]{EBD26B}34.4 &
  \cellcolor[HTML]{CACD72}26.8 \\ \cline{2-2}
\multirow{-3}{*}{A16} &
  F20 &
  \cellcolor[HTML]{E67C73}82.8 &
  \cellcolor[HTML]{E67C73}82.8 &
  \cellcolor[HTML]{E67C73}81.2 &
  \cellcolor[HTML]{E67C73}71.8 &
  \cellcolor[HTML]{E67C73}63.9 &
  \cellcolor[HTML]{E67C73}69.1 &
  \cellcolor[HTML]{E67C73}80.1 &
  \cellcolor[HTML]{E67C73}82.3 &
  \cellcolor[HTML]{B6CA76}22.3 &
  \cellcolor[HTML]{B0C977}21.0 &
  \cellcolor[HTML]{DBD06E}30.8 &
  \cellcolor[HTML]{D4CF70}29.1 &
  \cellcolor[HTML]{FFD366}39.2 &
  \cellcolor[HTML]{84C281}11.0 &
  \cellcolor[HTML]{E3D16C}32.5 &
  \cellcolor[HTML]{CCCD71}27.3 \\ \cline{1-2}
\end{tabular}%
}
\label{tab:expB}
\end{table*}


==> tex/table_features_explained.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|p{1cm}|p{1.8cm}|p{4.4cm}|p{8cm}|}
\hline
Feature ID & Occurrence Count & Feature Name                   & Feature Description                                                                     \\ \hline
F17 & 7 & loudness\_sma3\_stddevRisingSlope  & standard deviation of the rising slope of the simple moving average (with a window size of 3) of the loudness   \\ \hline
F19 & 7 & loudness\_sma3\_stddevFallingSlope & standard deviation of the falling slope of the simple moving average (with a window size of 3) of the loudness  \\ \hline
F66 & 6 & spectralFluxV\_sma3nz\_amean       & arithmetic mean of the simple moving average (with a window size of 3) of the spectral flux for non-zero values \\ \hline
F21 & 3 & spectralFlux\_sma3\_stddevNorm     & standard deviation-normalized simple moving average (with a window size of 3) of the spectral flux              \\ \hline
F12     & 2                                    & loudness\_sma3\_percentile20.0 & the 20th percentile of the simple moving average of the loudness values over 3 values   \\ \hline
F20     & 2                                    & spectralFlux\_sma3\_amean      & arithmetic mean of the simple moving average of spectral flux over a window of 3 values \\ \hline
F85     & 2                                    & MeanUnvoicedSegmentLength      & average length of all unvoiced segments within the audio file                           \\ \hline
F86     & 2                                    & StddevUnvoicedSegmentLength    & standard deviation of the length of all unvoiced segments within the audio file         \\ \hline
\end{tabular}%
\caption{Predictive Features and their interpretation}
\label{tab:feat-desc-table}
\end{table*}


==> tex/table_octav.tex <==

Octav: Testing imported table

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|l|l|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\cline{1-18} \cline{20-37}
 &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
   &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} \\
 &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   &
   &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} \\
\multirow{-3}{*}{Attack} &
  \multirow{-3}{*}{Feature} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A01}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A02}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A03}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A04}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A05}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A06}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A07}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A08}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A09}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A10}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A11}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A12}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A13}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A14}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A15}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A16}} &
   &
  \multirow{-3}{*}{Attack} &
  \multirow{-3}{*}{Feature} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A01}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A02}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A03}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A04}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A05}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A06}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A07}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A08}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A09}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A10}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A11}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A12}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A13}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A14}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A15}} &
  \multicolumn{1}{l|}{\multirow{-3}{*}{A16}} \\ \cline{1-18} \cline{20-37} 
 &
  F66 &
  \cellcolor[HTML]{88C280}12,8 &
  \cellcolor[HTML]{87C280}12,7 &
  \cellcolor[HTML]{94C47D}15,7 &
  \cellcolor[HTML]{ACC878}21,7 &
  \cellcolor[HTML]{D5CF6F}31,5 &
  \cellcolor[HTML]{BDCB75}25,7 &
  \cellcolor[HTML]{8BC37F}13,7 &
  \cellcolor[HTML]{9EC67B}18,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}69,5 &
  \cellcolor[HTML]{E67C73}68,1 &
  \cellcolor[HTML]{E67C73}70,3 &
  \cellcolor[HTML]{E67C73}60,0 &
  \cellcolor[HTML]{E67C73}55,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}76,2 &
   &
   &
  F86 &
  \cellcolor[HTML]{C7CD72}26,3 &
  \cellcolor[HTML]{B5CA76}22,3 &
  \cellcolor[HTML]{BDCB75}23,9 &
  \cellcolor[HTML]{D0CE71}28,2 &
  \cellcolor[HTML]{BACA75}23,3 &
  \cellcolor[HTML]{BECB74}24,2 &
  \cellcolor[HTML]{AEC978}20,6 &
  \cellcolor[HTML]{E77E72}49,8 &
  \cellcolor[HTML]{77C084}8,0 &
  \cellcolor[HTML]{74BF84}7,3 &
  \cellcolor[HTML]{E67C73}61,5 &
  \cellcolor[HTML]{FBD567}38,0 &
  \cellcolor[HTML]{E98571}49,0 &
  \cellcolor[HTML]{E67C73}65,0 &
  \cellcolor[HTML]{F1A16D}45,5 &
  \cellcolor[HTML]{F5B26B}43,3 \\ \cline{2-18} \cline{21-37} 
 &
  F19 &
  \cellcolor[HTML]{8CC37F}13,8 &
  \cellcolor[HTML]{89C380}13,0 &
  \cellcolor[HTML]{92C47E}15,3 &
  \cellcolor[HTML]{98C57C}16,8 &
  \cellcolor[HTML]{A3C77A}19,4 &
  \cellcolor[HTML]{99C57C}17,1 &
  \cellcolor[HTML]{9DC67B}17,8 &
  \cellcolor[HTML]{B2C977}23,0 &
  \cellcolor[HTML]{E67C73}61,9 &
  \cellcolor[HTML]{E67C73}62,8 &
  \cellcolor[HTML]{E67C73}55,7 &
  \cellcolor[HTML]{E67C73}78,7 &
  \cellcolor[HTML]{E67C73}54,7 &
  \cellcolor[HTML]{E67C73}54,5 &
  \cellcolor[HTML]{E67C73}65,3 &
  \cellcolor[HTML]{E67C73}66,7 &
   &
   &
  F85 &
  \cellcolor[HTML]{FCD567}38,3 &
  \cellcolor[HTML]{FDCD67}40,0 &
  \cellcolor[HTML]{F3D469}36,2 &
  \cellcolor[HTML]{FCD567}38,3 &
  \cellcolor[HTML]{F3D469}36,2 &
  \cellcolor[HTML]{F9D568}37,5 &
  \cellcolor[HTML]{D6CF6F}29,5 &
  \cellcolor[HTML]{E67C73}53,9 &
  \cellcolor[HTML]{86C280}11,5 &
  \cellcolor[HTML]{82C281}10,7 &
  \cellcolor[HTML]{E67C73}63,2 &
  \cellcolor[HTML]{ECD36A}34,7 &
  \cellcolor[HTML]{E67C73}68,0 &
  \cellcolor[HTML]{E67C73}97,0 &
  \cellcolor[HTML]{EE976F}46,8 &
  \cellcolor[HTML]{F2A56D}45,0 \\ \cline{2-18} \cline{21-37} 
\multirow{-3}{*}{A01} &
  F17 &
  \cellcolor[HTML]{90C47E}14,7 &
  \cellcolor[HTML]{8BC37F}13,6 &
  \cellcolor[HTML]{94C47D}15,8 &
  \cellcolor[HTML]{A8C879}20,5 &
  \cellcolor[HTML]{A5C77A}20,0 &
  \cellcolor[HTML]{A3C77A}19,3 &
  \cellcolor[HTML]{8FC47E}14,6 &
  \cellcolor[HTML]{A6C779}20,2 &
  \cellcolor[HTML]{E67C73}62,0 &
  \cellcolor[HTML]{E67C73}63,8 &
  \cellcolor[HTML]{E67C73}58,3 &
  \cellcolor[HTML]{E67C73}75,6 &
  \cellcolor[HTML]{E67C73}52,8 &
  \cellcolor[HTML]{E67C73}64,4 &
  \cellcolor[HTML]{E67C73}65,2 &
  \cellcolor[HTML]{E67C73}65,5 &
   &
  \multirow{-3}{*}{A09} &
  F12 &
  \cellcolor[HTML]{F1A16D}45,5 &
  \cellcolor[HTML]{F4AB6C}44,2 &
  \cellcolor[HTML]{EE966F}46,8 &
  \cellcolor[HTML]{F8BC69}42,1 &
  \cellcolor[HTML]{FED266}39,3 &
  \cellcolor[HTML]{FFD366}39,2 &
  \cellcolor[HTML]{FED567}38,7 &
  \cellcolor[HTML]{E67C73}65,0 &
  \cellcolor[HTML]{8BC37F}12,7 &
  \cellcolor[HTML]{89C380}12,2 &
  \cellcolor[HTML]{EB8D70}48,0 &
  \cellcolor[HTML]{FED266}39,3 &
  \cellcolor[HTML]{D4CF70}29,2 &
  \cellcolor[HTML]{A3C77A}18,2 &
  \cellcolor[HTML]{EFD36A}35,3 &
  \cellcolor[HTML]{F6D468}36,9 \\ \cline{1-18} \cline{20-37} 
 &
  F66 &
  \cellcolor[HTML]{88C280}12,8 &
  \cellcolor[HTML]{87C280}12,7 &
  \cellcolor[HTML]{94C47D}15,7 &
  \cellcolor[HTML]{ACC878}21,7 &
  \cellcolor[HTML]{D5CF6F}31,5 &
  \cellcolor[HTML]{BDCB75}25,7 &
  \cellcolor[HTML]{8BC37F}13,7 &
  \cellcolor[HTML]{9EC67B}18,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}69,5 &
  \cellcolor[HTML]{E67C73}68,1 &
  \cellcolor[HTML]{E67C73}70,3 &
  \cellcolor[HTML]{E67C73}60,0 &
  \cellcolor[HTML]{E67C73}55,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}76,2 &
   &
   &
  F86 &
  \cellcolor[HTML]{C7CD72}26,3 &
  \cellcolor[HTML]{B5CA76}22,3 &
  \cellcolor[HTML]{BDCB75}23,9 &
  \cellcolor[HTML]{D0CE71}28,2 &
  \cellcolor[HTML]{BACA75}23,3 &
  \cellcolor[HTML]{BECB74}24,2 &
  \cellcolor[HTML]{AEC978}20,6 &
  \cellcolor[HTML]{E77E72}49,8 &
  \cellcolor[HTML]{77C084}8,0 &
  \cellcolor[HTML]{74BF84}7,3 &
  \cellcolor[HTML]{E67C73}61,5 &
  \cellcolor[HTML]{FBD567}38,0 &
  \cellcolor[HTML]{E98571}49,0 &
  \cellcolor[HTML]{E67C73}65,0 &
  \cellcolor[HTML]{F1A16D}45,5 &
  \cellcolor[HTML]{F2A56D}45,0 \\ \cline{2-18} \cline{21-37} 
 &
  F19 &
  \cellcolor[HTML]{8CC37F}13,8 &
  \cellcolor[HTML]{89C380}13,0 &
  \cellcolor[HTML]{92C47E}15,3 &
  \cellcolor[HTML]{98C57C}16,8 &
  \cellcolor[HTML]{A3C77A}19,4 &
  \cellcolor[HTML]{99C57C}17,1 &
  \cellcolor[HTML]{9DC67B}17,8 &
  \cellcolor[HTML]{B2C977}23,0 &
  \cellcolor[HTML]{E67C73}61,9 &
  \cellcolor[HTML]{E67C73}62,8 &
  \cellcolor[HTML]{E67C73}55,7 &
  \cellcolor[HTML]{E67C73}78,7 &
  \cellcolor[HTML]{E67C73}54,7 &
  \cellcolor[HTML]{E67C73}54,5 &
  \cellcolor[HTML]{E67C73}65,3 &
  \cellcolor[HTML]{E67C73}66,7 &
   &
   &
  F85 &
  \cellcolor[HTML]{FCD567}38,3 &
  \cellcolor[HTML]{FDCD67}40,0 &
  \cellcolor[HTML]{F3D469}36,2 &
  \cellcolor[HTML]{FCD567}38,3 &
  \cellcolor[HTML]{F3D469}36,2 &
  \cellcolor[HTML]{F9D568}37,5 &
  \cellcolor[HTML]{D6CF6F}29,5 &
  \cellcolor[HTML]{E67C73}53,9 &
  \cellcolor[HTML]{86C280}11,5 &
  \cellcolor[HTML]{82C281}10,7 &
  \cellcolor[HTML]{E67C73}63,2 &
  \cellcolor[HTML]{ECD36A}34,7 &
  \cellcolor[HTML]{E67C73}68,0 &
  \cellcolor[HTML]{E67C73}97,0 &
  \cellcolor[HTML]{EE976F}46,8 &
  \cellcolor[HTML]{F5B26B}43,3 \\ \cline{2-18} \cline{21-37} 
\multirow{-3}{*}{A02} &
  F17 &
  \cellcolor[HTML]{90C47E}14,7 &
  \cellcolor[HTML]{8BC37F}13,6 &
  \cellcolor[HTML]{94C47D}15,8 &
  \cellcolor[HTML]{A8C879}20,5 &
  \cellcolor[HTML]{A5C77A}20,0 &
  \cellcolor[HTML]{A3C77A}19,3 &
  \cellcolor[HTML]{8FC47E}14,6 &
  \cellcolor[HTML]{A6C779}20,2 &
  \cellcolor[HTML]{E67C73}62,0 &
  \cellcolor[HTML]{E67C73}63,8 &
  \cellcolor[HTML]{E67C73}58,3 &
  \cellcolor[HTML]{E67C73}75,6 &
  \cellcolor[HTML]{E67C73}52,8 &
  \cellcolor[HTML]{E67C73}64,4 &
  \cellcolor[HTML]{E67C73}65,2 &
  \cellcolor[HTML]{E67C73}65,5 &
   &
  \multirow{-3}{*}{A10} &
  F12 &
  \cellcolor[HTML]{F1A16D}45,5 &
  \cellcolor[HTML]{F4AB6C}44,2 &
  \cellcolor[HTML]{EE966F}46,8 &
  \cellcolor[HTML]{F8BC69}42,1 &
  \cellcolor[HTML]{FED266}39,3 &
  \cellcolor[HTML]{FFD366}39,2 &
  \cellcolor[HTML]{FED567}38,7 &
  \cellcolor[HTML]{E67C73}65,0 &
  \cellcolor[HTML]{8BC37F}12,7 &
  \cellcolor[HTML]{89C380}12,2 &
  \cellcolor[HTML]{EB8D70}48,0 &
  \cellcolor[HTML]{FED266}39,3 &
  \cellcolor[HTML]{D4CF70}29,2 &
  \cellcolor[HTML]{A3C77A}18,2 &
  \cellcolor[HTML]{EFD36A}35,3 &
  \cellcolor[HTML]{F6D468}36,9 \\ \cline{1-18} \cline{20-37} 
 &
  F19 &
  \cellcolor[HTML]{8CC37F}13,8 &
  \cellcolor[HTML]{89C380}13,0 &
  \cellcolor[HTML]{92C47E}15,3 &
  \cellcolor[HTML]{98C57C}16,8 &
  \cellcolor[HTML]{A3C77A}19,4 &
  \cellcolor[HTML]{99C57C}17,1 &
  \cellcolor[HTML]{9DC67B}17,8 &
  \cellcolor[HTML]{B2C977}23,0 &
  \cellcolor[HTML]{E67C73}61,9 &
  \cellcolor[HTML]{E67C73}62,8 &
  \cellcolor[HTML]{E67C73}55,7 &
  \cellcolor[HTML]{E67C73}78,7 &
  \cellcolor[HTML]{E67C73}54,7 &
  \cellcolor[HTML]{E67C73}54,5 &
  \cellcolor[HTML]{E67C73}65,3 &
  \cellcolor[HTML]{E67C73}66,7 &
   &
   &
  F58 &
  \cellcolor[HTML]{EA8871}48,6 &
  \cellcolor[HTML]{E67C73}50,3 &
  \cellcolor[HTML]{E88372}49,3 &
  \cellcolor[HTML]{E88272}49,3 &
  \cellcolor[HTML]{F3AA6C}44,3 &
  \cellcolor[HTML]{F7B76A}42,7 &
  \cellcolor[HTML]{FAC169}41,4 &
  \cellcolor[HTML]{EB8D70}48,0 &
  \cellcolor[HTML]{F4D469}36,5 &
  \cellcolor[HTML]{FCD567}38,2 &
  \cellcolor[HTML]{97C57D}15,3 &
  \cellcolor[HTML]{E67C73}51,3 &
  \cellcolor[HTML]{E67C73}50,8 &
  \cellcolor[HTML]{E67C73}54,8 &
  \cellcolor[HTML]{FFD566}38,9 &
  \cellcolor[HTML]{E77F72}49,7 \\ \cline{2-18} \cline{21-37} 
 &
  F66 &
  \cellcolor[HTML]{88C280}12,8 &
  \cellcolor[HTML]{87C280}12,7 &
  \cellcolor[HTML]{94C47D}15,7 &
  \cellcolor[HTML]{ACC878}21,7 &
  \cellcolor[HTML]{D5CF6F}31,5 &
  \cellcolor[HTML]{BDCB75}25,7 &
  \cellcolor[HTML]{8BC37F}13,7 &
  \cellcolor[HTML]{9EC67B}18,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}69,5 &
  \cellcolor[HTML]{E67C73}68,1 &
  \cellcolor[HTML]{E67C73}70,3 &
  \cellcolor[HTML]{E67C73}60,0 &
  \cellcolor[HTML]{E67C73}55,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}76,2 &
   &
   &
  F60 &
  \cellcolor[HTML]{EF9B6E}46,2 &
  \cellcolor[HTML]{EB8D70}48,0 &
  \cellcolor[HTML]{EF9D6E}46,0 &
  \cellcolor[HTML]{E98671}48,8 &
  \cellcolor[HTML]{F5B16B}43,5 &
  \cellcolor[HTML]{FBC768}40,7 &
  \cellcolor[HTML]{FCCB67}40,3 &
  \cellcolor[HTML]{EF9B6E}46,3 &
  \cellcolor[HTML]{F0D36A}35,6 &
  \cellcolor[HTML]{FAD567}37,8 &
  \cellcolor[HTML]{97C57D}15,3 &
  \cellcolor[HTML]{E67C73}52,6 &
  \cellcolor[HTML]{E98571}49,0 &
  \cellcolor[HTML]{E67C73}58,7 &
  \cellcolor[HTML]{F8D468}37,3 &
  \cellcolor[HTML]{FBC768}40,7 \\ \cline{2-18} \cline{21-37} 
\multirow{-3}{*}{A03} &
  F17 &
  \cellcolor[HTML]{90C47E}14,7 &
  \cellcolor[HTML]{8BC37F}13,6 &
  \cellcolor[HTML]{94C47D}15,8 &
  \cellcolor[HTML]{A8C879}20,5 &
  \cellcolor[HTML]{A5C77A}20,0 &
  \cellcolor[HTML]{A3C77A}19,3 &
  \cellcolor[HTML]{8FC47E}14,6 &
  \cellcolor[HTML]{A6C779}20,2 &
  \cellcolor[HTML]{E67C73}62,0 &
  \cellcolor[HTML]{E67C73}63,8 &
  \cellcolor[HTML]{E67C73}58,3 &
  \cellcolor[HTML]{E67C73}75,6 &
  \cellcolor[HTML]{E67C73}52,8 &
  \cellcolor[HTML]{E67C73}64,4 &
  \cellcolor[HTML]{E67C73}65,2 &
  \cellcolor[HTML]{E67C73}65,5 &
   &
  \multirow{-3}{*}{A11} &
  F59 &
  \cellcolor[HTML]{FDCE67}39,8 &
  \cellcolor[HTML]{F8D468}37,3 &
  \cellcolor[HTML]{FCC967}40,5 &
  \cellcolor[HTML]{EA8A71}48,3 &
  \cellcolor[HTML]{FFD366}39,2 &
  \cellcolor[HTML]{F8D468}37,3 &
  \cellcolor[HTML]{E1D16D}32,2 &
  \cellcolor[HTML]{F9BF69}41,7 &
  \cellcolor[HTML]{FED567}38,6 &
  \cellcolor[HTML]{FAC169}41,4 &
  \cellcolor[HTML]{A1C77A}17,7 &
  \cellcolor[HTML]{E67C73}50,5 &
  \cellcolor[HTML]{D3CE70}28,8 &
  \cellcolor[HTML]{87C280}11,8 &
  \cellcolor[HTML]{F4D469}36,5 &
  \cellcolor[HTML]{F9C169}41,5 \\ \cline{1-18} \cline{20-37} 
 &
  F19 &
  \cellcolor[HTML]{8CC37F}13,8 &
  \cellcolor[HTML]{89C380}13,0 &
  \cellcolor[HTML]{92C47E}15,3 &
  \cellcolor[HTML]{98C57C}16,8 &
  \cellcolor[HTML]{A3C77A}19,4 &
  \cellcolor[HTML]{99C57C}17,1 &
  \cellcolor[HTML]{9DC67B}17,8 &
  \cellcolor[HTML]{B2C977}23,0 &
  \cellcolor[HTML]{E67C73}61,9 &
  \cellcolor[HTML]{E67C73}62,8 &
  \cellcolor[HTML]{E67C73}55,7 &
  \cellcolor[HTML]{E67C73}78,7 &
  \cellcolor[HTML]{E67C73}54,7 &
  \cellcolor[HTML]{E67C73}54,5 &
  \cellcolor[HTML]{E67C73}65,3 &
  \cellcolor[HTML]{E67C73}66,7 &
   &
   &
  F82 &
  \cellcolor[HTML]{EAD26B}34,1 &
  \cellcolor[HTML]{E7D26B}33,6 &
  \cellcolor[HTML]{F3D469}36,2 &
  \cellcolor[HTML]{D5CF6F}29,3 &
  \cellcolor[HTML]{D6CF6F}29,6 &
  \cellcolor[HTML]{D2CE70}28,7 &
  \cellcolor[HTML]{EC9070}47,6 &
  \cellcolor[HTML]{E67C73}60,2 &
  \cellcolor[HTML]{F5D469}36,6 &
  \cellcolor[HTML]{EBD26B}34,3 &
  \cellcolor[HTML]{E67C73}64,5 &
  \cellcolor[HTML]{A3C77A}18,2 &
  \cellcolor[HTML]{E67C73}66,1 &
  \cellcolor[HTML]{E67C73}94,0 &
  \cellcolor[HTML]{F6B36B}43,2 &
  \cellcolor[HTML]{E67C73}51,3 \\ \cline{2-18} \cline{21-37} 
 &
  F21 &
  \cellcolor[HTML]{ADC878}21,9 &
  \cellcolor[HTML]{ACC878}21,6 &
  \cellcolor[HTML]{B9CA75}24,8 &
  \cellcolor[HTML]{9BC57C}17,3 &
  \cellcolor[HTML]{9BC67C}17,5 &
  \cellcolor[HTML]{98C57C}16,8 &
  \cellcolor[HTML]{A0C67B}18,7 &
  \cellcolor[HTML]{F4AC6C}45,7 &
  \cellcolor[HTML]{9EC67B}18,1 &
  \cellcolor[HTML]{9BC67C}17,5 &
  \cellcolor[HTML]{F7D468}40,0 &
  \cellcolor[HTML]{FAC169}43,7 &
  \cellcolor[HTML]{DED06D}33,8 &
  \cellcolor[HTML]{C9CD72}28,6 &
  \cellcolor[HTML]{E9D26B}36,5 &
  \cellcolor[HTML]{FED567}41,5 &
   &
   &
  F19 &
  \cellcolor[HTML]{E67C73}86,2 &
  \cellcolor[HTML]{E67C73}87,0 &
  \cellcolor[HTML]{E67C73}84,7 &
  \cellcolor[HTML]{E67C73}83,3 &
  \cellcolor[HTML]{E67C73}80,6 &
  \cellcolor[HTML]{E67C73}82,9 &
  \cellcolor[HTML]{E67C73}82,2 &
  \cellcolor[HTML]{E67C73}77,0 &
  \cellcolor[HTML]{FBD567}38,1 &
  \cellcolor[HTML]{F8D468}37,3 &
  \cellcolor[HTML]{F3AA6C}44,3 &
  \cellcolor[HTML]{B1C977}21,3 &
  \cellcolor[HTML]{F1A26D}45,3 &
  \cellcolor[HTML]{F1A16D}45,5 &
  \cellcolor[HTML]{EDD36A}34,8 &
  \cellcolor[HTML]{E6D26C}33,3 \\ \cline{2-18} \cline{21-37} 
\multirow{-3}{*}{A04} &
  F81 &
  \cellcolor[HTML]{D1CE70}30,5 &
  \cellcolor[HTML]{D6CF6F}31,8 &
  \cellcolor[HTML]{DBD06E}33,2 &
  \cellcolor[HTML]{A6C77A}20,1 &
  \cellcolor[HTML]{B7CA76}24,3 &
  \cellcolor[HTML]{B9CA75}24,8 &
  \cellcolor[HTML]{D7CF6F}32,0 &
  \cellcolor[HTML]{E67C73}59,0 &
  \cellcolor[HTML]{B0C977}22,5 &
  \cellcolor[HTML]{AAC879}21,2 &
  \cellcolor[HTML]{E67C73}52,8 &
  \cellcolor[HTML]{C7CD72}28,2 &
  \cellcolor[HTML]{FCC868}43,0 &
  \cellcolor[HTML]{D6CF6F}31,8 &
  \cellcolor[HTML]{FDD567}41,4 &
  \cellcolor[HTML]{F2D369}38,6 &
   &
  \multirow{-3}{*}{A12} &
  F83 &
  \cellcolor[HTML]{FBC768}40,7 &
  \cellcolor[HTML]{FFD366}39,2 &
  \cellcolor[HTML]{F2A56D}45,0 &
  \cellcolor[HTML]{E5D16C}33,1 &
  \cellcolor[HTML]{F7D468}37,2 &
  \cellcolor[HTML]{EED36A}35,0 &
  \cellcolor[HTML]{E67C73}61,4 &
  \cellcolor[HTML]{E67C73}56,5 &
  \cellcolor[HTML]{E67C73}61,3 &
  \cellcolor[HTML]{E67C73}60,7 &
  \cellcolor[HTML]{EA8971}48,5 &
  \cellcolor[HTML]{B8CA76}22,8 &
  \cellcolor[HTML]{EED36A}35,2 &
  \cellcolor[HTML]{5BBB89}1,8 &
  \cellcolor[HTML]{F6B36B}43,2 &
  \cellcolor[HTML]{E67C73}55,1 \\ \cline{1-18} \cline{20-37} 
 &
  F21 &
  \cellcolor[HTML]{ADC878}21,9 &
  \cellcolor[HTML]{ACC878}21,6 &
  \cellcolor[HTML]{B9CA75}24,8 &
  \cellcolor[HTML]{9BC57C}17,3 &
  \cellcolor[HTML]{9BC67C}17,5 &
  \cellcolor[HTML]{98C57C}16,8 &
  \cellcolor[HTML]{A0C67B}18,7 &
  \cellcolor[HTML]{F4AC6C}45,7 &
  \cellcolor[HTML]{9EC67B}18,1 &
  \cellcolor[HTML]{9BC67C}17,5 &
  \cellcolor[HTML]{F7D468}40,0 &
  \cellcolor[HTML]{FAC169}43,7 &
  \cellcolor[HTML]{DED06D}33,8 &
  \cellcolor[HTML]{C9CD72}28,6 &
  \cellcolor[HTML]{E9D26B}36,5 &
  \cellcolor[HTML]{FED567}41,5 &
   &
   &
  F67 &
  \cellcolor[HTML]{E1D16D}32,0 &
  \cellcolor[HTML]{DAD06E}30,6 &
  \cellcolor[HTML]{EAD26B}34,1 &
  \cellcolor[HTML]{C2CC74}25,0 &
  \cellcolor[HTML]{C0CB74}24,6 &
  \cellcolor[HTML]{C3CC73}25,3 &
  \cellcolor[HTML]{C1CC74}24,8 &
  \cellcolor[HTML]{FFD566}39,0 &
  \cellcolor[HTML]{FBC768}40,7 &
  \cellcolor[HTML]{FECF67}39,7 &
  \cellcolor[HTML]{E6D26C}33,2 &
  \cellcolor[HTML]{E88172}49,5 &
  \cellcolor[HTML]{B5CA76}22,1 &
  \cellcolor[HTML]{95C57D}15,0 &
  \cellcolor[HTML]{FBD567}38,1 &
  \cellcolor[HTML]{F1D369}35,8 \\ \cline{2-18} \cline{21-37} 
 &
  F19 &
  \cellcolor[HTML]{8CC37F}13,8 &
  \cellcolor[HTML]{89C380}13,0 &
  \cellcolor[HTML]{92C47E}15,3 &
  \cellcolor[HTML]{98C57C}16,8 &
  \cellcolor[HTML]{A3C77A}19,4 &
  \cellcolor[HTML]{99C57C}17,1 &
  \cellcolor[HTML]{9DC67B}17,8 &
  \cellcolor[HTML]{B2C977}23,0 &
  \cellcolor[HTML]{E67C73}61,9 &
  \cellcolor[HTML]{E67C73}62,8 &
  \cellcolor[HTML]{E67C73}55,7 &
  \cellcolor[HTML]{E67C73}78,7 &
  \cellcolor[HTML]{E67C73}54,7 &
  \cellcolor[HTML]{E67C73}54,5 &
  \cellcolor[HTML]{E67C73}65,3 &
  \cellcolor[HTML]{E67C73}66,7 &
   &
   &
  F39 &
  \cellcolor[HTML]{F3D469}36,1 &
  \cellcolor[HTML]{E6D26C}33,3 &
  \cellcolor[HTML]{F8D468}37,3 &
  \cellcolor[HTML]{F7B96A}42,5 &
  \cellcolor[HTML]{E8D26B}33,7 &
  \cellcolor[HTML]{E7D26C}33,4 &
  \cellcolor[HTML]{C5CC73}25,8 &
  \cellcolor[HTML]{FBD567}37,9 &
  \cellcolor[HTML]{FDD567}38,4 &
  \cellcolor[HTML]{FCC967}40,5 &
  \cellcolor[HTML]{D2CE70}28,7 &
  \cellcolor[HTML]{E88272}49,3 &
  \cellcolor[HTML]{B8CA76}22,8 &
  \cellcolor[HTML]{ACC878}20,1 &
  \cellcolor[HTML]{F6D468}36,8 &
  \cellcolor[HTML]{E5D16C}33,0 \\ \cline{2-18} \cline{21-37} 
\multirow{-3}{*}{A05} &
  F17 &
  \cellcolor[HTML]{90C47E}14,7 &
  \cellcolor[HTML]{8BC37F}13,6 &
  \cellcolor[HTML]{94C47D}15,8 &
  \cellcolor[HTML]{A8C879}20,5 &
  \cellcolor[HTML]{A5C77A}20,0 &
  \cellcolor[HTML]{A3C77A}19,3 &
  \cellcolor[HTML]{8FC47E}14,6 &
  \cellcolor[HTML]{A6C779}20,2 &
  \cellcolor[HTML]{E67C73}62,0 &
  \cellcolor[HTML]{E67C73}63,8 &
  \cellcolor[HTML]{E67C73}58,3 &
  \cellcolor[HTML]{E67C73}75,6 &
  \cellcolor[HTML]{E67C73}52,8 &
  \cellcolor[HTML]{E67C73}64,4 &
  \cellcolor[HTML]{E67C73}65,2 &
  \cellcolor[HTML]{E67C73}65,5 &
   &
  \multirow{-3}{*}{A13} &
  F49 &
  \cellcolor[HTML]{F3AB6C}44,3 &
  \cellcolor[HTML]{F8BA6A}42,3 &
  \cellcolor[HTML]{F09E6E}45,8 &
  \cellcolor[HTML]{E67C73}51,3 &
  \cellcolor[HTML]{EB8E70}47,8 &
  \cellcolor[HTML]{E98671}48,8 &
  \cellcolor[HTML]{F9BF69}41,8 &
  \cellcolor[HTML]{E98671}48,8 &
  \cellcolor[HTML]{EC9170}47,5 &
  \cellcolor[HTML]{E88272}49,3 &
  \cellcolor[HTML]{FBC768}40,8 &
  \cellcolor[HTML]{EC926F}47,3 &
  \cellcolor[HTML]{C2CC74}25,0 &
  \cellcolor[HTML]{B7CA76}22,6 &
  \cellcolor[HTML]{FAC268}41,3 &
  \cellcolor[HTML]{FAC268}41,3 \\ \cline{1-18} \cline{20-37} 
 &
  F21 &
  \cellcolor[HTML]{ADC878}21,9 &
  \cellcolor[HTML]{ACC878}21,6 &
  \cellcolor[HTML]{B9CA75}24,8 &
  \cellcolor[HTML]{9BC57C}17,3 &
  \cellcolor[HTML]{9BC67C}17,5 &
  \cellcolor[HTML]{98C57C}16,8 &
  \cellcolor[HTML]{A0C67B}18,7 &
  \cellcolor[HTML]{F4AC6C}45,7 &
  \cellcolor[HTML]{9EC67B}18,1 &
  \cellcolor[HTML]{9BC67C}17,5 &
  \cellcolor[HTML]{F7D468}40,0 &
  \cellcolor[HTML]{FAC169}43,7 &
  \cellcolor[HTML]{DED06D}33,8 &
  \cellcolor[HTML]{C9CD72}28,6 &
  \cellcolor[HTML]{E9D26B}36,5 &
  \cellcolor[HTML]{FED567}41,5 &
   &
   &
  F45 &
  \cellcolor[HTML]{E67C73}52,8 &
  \cellcolor[HTML]{E67C73}53,3 &
  \cellcolor[HTML]{E67C73}56,9 &
  \cellcolor[HTML]{EF9C6E}46,7 &
  \cellcolor[HTML]{E67C73}50,4 &
  \cellcolor[HTML]{EC8F70}48,1 &
  \cellcolor[HTML]{E67C73}71,2 &
  \cellcolor[HTML]{E67C73}55,6 &
  \cellcolor[HTML]{E67C73}80,9 &
  \cellcolor[HTML]{E67C73}80,8 &
  \cellcolor[HTML]{FCD567}39,9 &
  \cellcolor[HTML]{FCCA67}41,8 &
  \cellcolor[HTML]{DBD06E}32,1 &
  \cellcolor[HTML]{57BB8A}0,8 &
  \cellcolor[HTML]{F2A66C}45,6 &
  \cellcolor[HTML]{E67C73}55,0 \\ \cline{2-18} \cline{21-37} 
 &
  F19 &
  \cellcolor[HTML]{8CC37F}13,8 &
  \cellcolor[HTML]{89C380}13,0 &
  \cellcolor[HTML]{92C47E}15,3 &
  \cellcolor[HTML]{98C57C}16,8 &
  \cellcolor[HTML]{A3C77A}19,4 &
  \cellcolor[HTML]{99C57C}17,1 &
  \cellcolor[HTML]{9DC67B}17,8 &
  \cellcolor[HTML]{B2C977}23,0 &
  \cellcolor[HTML]{E67C73}61,9 &
  \cellcolor[HTML]{E67C73}62,8 &
  \cellcolor[HTML]{E67C73}55,7 &
  \cellcolor[HTML]{E67C73}78,7 &
  \cellcolor[HTML]{E67C73}54,7 &
  \cellcolor[HTML]{E67C73}54,5 &
  \cellcolor[HTML]{E67C73}65,3 &
  \cellcolor[HTML]{E67C73}66,7 &
   &
   &
  F51 &
  \cellcolor[HTML]{E67C73}51,0 &
  \cellcolor[HTML]{E67C73}51,0 &
  \cellcolor[HTML]{E67C73}54,3 &
  \cellcolor[HTML]{F4AD6B}44,8 &
  \cellcolor[HTML]{F3AA6C}45,2 &
  \cellcolor[HTML]{FBC668}42,3 &
  \cellcolor[HTML]{E67C73}65,0 &
  \cellcolor[HTML]{E67C73}53,2 &
  \cellcolor[HTML]{E67C73}73,8 &
  \cellcolor[HTML]{E67C73}73,8 &
  \cellcolor[HTML]{E5D16C}34,3 &
  \cellcolor[HTML]{F9BF69}43,0 &
  \cellcolor[HTML]{CFCE71}29,3 &
  \cellcolor[HTML]{57BB8A}0,8 &
  \cellcolor[HTML]{FBC868}42,0 &
  \cellcolor[HTML]{E67C73}56,0 \\ \cline{2-18} \cline{21-37} 
\multirow{-3}{*}{A06} &
  F17 &
  \cellcolor[HTML]{90C47E}14,7 &
  \cellcolor[HTML]{8BC37F}13,6 &
  \cellcolor[HTML]{94C47D}15,8 &
  \cellcolor[HTML]{A8C879}20,5 &
  \cellcolor[HTML]{A5C77A}20,0 &
  \cellcolor[HTML]{A3C77A}19,3 &
  \cellcolor[HTML]{8FC47E}14,6 &
  \cellcolor[HTML]{A6C779}20,2 &
  \cellcolor[HTML]{E67C73}62,0 &
  \cellcolor[HTML]{E67C73}63,8 &
  \cellcolor[HTML]{E67C73}58,3 &
  \cellcolor[HTML]{E67C73}75,6 &
  \cellcolor[HTML]{E67C73}52,8 &
  \cellcolor[HTML]{E67C73}64,4 &
  \cellcolor[HTML]{E67C73}65,2 &
  \cellcolor[HTML]{E67C73}65,5 &
   &
  \multirow{-3}{*}{A14} &
  F57 &
  \cellcolor[HTML]{E88172}49,5 &
  \cellcolor[HTML]{EB8E70}48,2 &
  \cellcolor[HTML]{E67C73}52,2 &
  \cellcolor[HTML]{F7B76A}43,8 &
  \cellcolor[HTML]{F8BA6A}43,5 &
  \cellcolor[HTML]{FED567}40,4 &
  \cellcolor[HTML]{E67C73}62,5 &
  \cellcolor[HTML]{E67C73}51,3 &
  \cellcolor[HTML]{E67C73}70,0 &
  \cellcolor[HTML]{E67C73}71,0 &
  \cellcolor[HTML]{DCD06E}32,3 &
  \cellcolor[HTML]{FBC568}42,3 &
  \cellcolor[HTML]{C1CC74}25,8 &
  \cellcolor[HTML]{57BB8A}0,8 &
  \cellcolor[HTML]{F8D568}39,0 &
  \cellcolor[HTML]{E67C73}51,7 \\ \cline{1-18} \cline{20-37} 
 &
  F66 &
  \cellcolor[HTML]{88C280}12,8 &
  \cellcolor[HTML]{87C280}12,7 &
  \cellcolor[HTML]{94C47D}15,7 &
  \cellcolor[HTML]{ACC878}21,7 &
  \cellcolor[HTML]{D5CF6F}31,5 &
  \cellcolor[HTML]{BDCB75}25,7 &
  \cellcolor[HTML]{8BC37F}13,7 &
  \cellcolor[HTML]{9EC67B}18,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}69,5 &
  \cellcolor[HTML]{E67C73}68,1 &
  \cellcolor[HTML]{E67C73}70,3 &
  \cellcolor[HTML]{E67C73}60,0 &
  \cellcolor[HTML]{E67C73}55,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}76,2 &
   &
   &
  F78 &
  \cellcolor[HTML]{E67C73}56,2 &
  \cellcolor[HTML]{E67C73}59,7 &
  \cellcolor[HTML]{E67C73}57,7 &
  \cellcolor[HTML]{E67C73}55,7 &
  \cellcolor[HTML]{E67C73}52,2 &
  \cellcolor[HTML]{E67C73}53,2 &
  \cellcolor[HTML]{E67C73}57,8 &
  \cellcolor[HTML]{EA8771}49,0 &
  \cellcolor[HTML]{FBC768}43,2 &
  \cellcolor[HTML]{F7B66A}44,7 &
  \cellcolor[HTML]{FCD567}41,2 &
  \cellcolor[HTML]{E67C73}51,8 &
  \cellcolor[HTML]{E67C73}62,7 &
  \cellcolor[HTML]{E67C73}58,5 &
  \cellcolor[HTML]{A8C879}20,7 &
  \cellcolor[HTML]{F5AF6B}45,3 \\ \cline{2-18} \cline{21-37} 
 &
  F1 &
  \cellcolor[HTML]{DAD06E}32,9 &
  \cellcolor[HTML]{D3CE70}31,0 &
  \cellcolor[HTML]{CCCD71}29,5 &
  \cellcolor[HTML]{EBD26B}37,0 &
  \cellcolor[HTML]{CACD72}29,0 &
  \cellcolor[HTML]{D9D06E}32,7 &
  \cellcolor[HTML]{8EC37F}14,2 &
  \cellcolor[HTML]{E1D16D}34,4 &
  \cellcolor[HTML]{E2D16D}34,8 &
  \cellcolor[HTML]{E0D16D}34,3 &
  \cellcolor[HTML]{E67C73}50,7 &
  \cellcolor[HTML]{E88172}49,6 &
  \cellcolor[HTML]{CACD72}28,8 &
  \cellcolor[HTML]{A7C779}20,3 &
  \cellcolor[HTML]{DED06D}33,8 &
  \cellcolor[HTML]{E5D16C}35,6 &
   &
   &
  F77 &
  \cellcolor[HTML]{E88172}49,6 &
  \cellcolor[HTML]{E77F72}49,8 &
  \cellcolor[HTML]{E67C73}50,3 &
  \cellcolor[HTML]{EA8971}48,8 &
  \cellcolor[HTML]{ED926F}48,0 &
  \cellcolor[HTML]{EE976F}47,6 &
  \cellcolor[HTML]{E67C73}55,3 &
  \cellcolor[HTML]{F5B16B}45,2 &
  \cellcolor[HTML]{EC9070}48,2 &
  \cellcolor[HTML]{EA8871}48,9 &
  \cellcolor[HTML]{B0C977}22,6 &
  \cellcolor[HTML]{F3A86C}46,0 &
  \cellcolor[HTML]{E67C73}58,3 &
  \cellcolor[HTML]{D4CF70}31,3 &
  \cellcolor[HTML]{BDCB75}25,7 &
  \cellcolor[HTML]{F9BF69}43,8 \\ \cline{2-18} \cline{21-37} 
\multirow{-3}{*}{A07} &
  F17 &
  \cellcolor[HTML]{90C47E}14,7 &
  \cellcolor[HTML]{8BC37F}13,6 &
  \cellcolor[HTML]{94C47D}15,8 &
  \cellcolor[HTML]{A8C879}20,5 &
  \cellcolor[HTML]{A5C77A}20,0 &
  \cellcolor[HTML]{A3C77A}19,3 &
  \cellcolor[HTML]{8FC47E}14,6 &
  \cellcolor[HTML]{A6C779}20,2 &
  \cellcolor[HTML]{E67C73}62,0 &
  \cellcolor[HTML]{E67C73}63,8 &
  \cellcolor[HTML]{E67C73}58,3 &
  \cellcolor[HTML]{E67C73}75,6 &
  \cellcolor[HTML]{E67C73}52,8 &
  \cellcolor[HTML]{E67C73}64,4 &
  \cellcolor[HTML]{E67C73}65,2 &
  \cellcolor[HTML]{E67C73}65,5 &
   &
  \multirow{-3}{*}{A15} &
  F76 &
  \cellcolor[HTML]{E77E72}49,8 &
  \cellcolor[HTML]{E67C73}50,3 &
  \cellcolor[HTML]{E67C73}51,7 &
  \cellcolor[HTML]{E67C73}51,0 &
  \cellcolor[HTML]{EB8D70}48,5 &
  \cellcolor[HTML]{EA8971}48,8 &
  \cellcolor[HTML]{E67C73}57,3 &
  \cellcolor[HTML]{F2A66C}46,2 &
  \cellcolor[HTML]{F1A16D}46,7 &
  \cellcolor[HTML]{EF996E}47,3 &
  \cellcolor[HTML]{ACC878}21,7 &
  \cellcolor[HTML]{F5B26B}45,1 &
  \cellcolor[HTML]{E67C73}57,2 &
  \cellcolor[HTML]{D7CF6F}32,0 &
  \cellcolor[HTML]{C1CC74}26,8 &
  \cellcolor[HTML]{E67C73}54,9 \\ \cline{1-18} \cline{20-37} 
 &
  F20 &
  \cellcolor[HTML]{9AC57C}17,2 &
  \cellcolor[HTML]{9AC57C}17,2 &
  \cellcolor[HTML]{A1C67B}18,8 &
  \cellcolor[HTML]{C7CD72}28,2 &
  \cellcolor[HTML]{E7D26B}36,1 &
  \cellcolor[HTML]{D2CE70}30,9 &
  \cellcolor[HTML]{A5C77A}19,9 &
  \cellcolor[HTML]{9CC67C}17,7 &
  \cellcolor[HTML]{E67C73}77,7 &
  \cellcolor[HTML]{E67C73}79,0 &
  \cellcolor[HTML]{E67C73}69,2 &
  \cellcolor[HTML]{E67C73}70,9 &
  \cellcolor[HTML]{E67C73}60,8 &
  \cellcolor[HTML]{E67C73}89,0 &
  \cellcolor[HTML]{E67C73}67,5 &
  \cellcolor[HTML]{E67C73}72,7 &
   &
   &
  F66 &
  \cellcolor[HTML]{E67C73}87,2 &
  \cellcolor[HTML]{E67C73}87,3 &
  \cellcolor[HTML]{E67C73}84,3 &
  \cellcolor[HTML]{E67C73}78,3 &
  \cellcolor[HTML]{E67C73}68,5 &
  \cellcolor[HTML]{E67C73}74,3 &
  \cellcolor[HTML]{E67C73}86,3 &
  \cellcolor[HTML]{E67C73}81,8 &
  \cellcolor[HTML]{DED06E}31,3 &
  \cellcolor[HTML]{DAD06E}30,5 &
  \cellcolor[HTML]{E0D16D}31,9 &
  \cellcolor[HTML]{D6CF6F}29,7 &
  \cellcolor[HTML]{FDCD67}40,0 &
  \cellcolor[HTML]{F2A66D}44,8 &
  \cellcolor[HTML]{DED06E}31,3 &
  \cellcolor[HTML]{BCCB75}23,8 \\ \cline{2-18} \cline{21-37} 
 &
  F66 &
  \cellcolor[HTML]{88C280}12,8 &
  \cellcolor[HTML]{87C280}12,7 &
  \cellcolor[HTML]{94C47D}15,7 &
  \cellcolor[HTML]{ACC878}21,7 &
  \cellcolor[HTML]{D5CF6F}31,5 &
  \cellcolor[HTML]{BDCB75}25,7 &
  \cellcolor[HTML]{8BC37F}13,7 &
  \cellcolor[HTML]{9EC67B}18,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}69,5 &
  \cellcolor[HTML]{E67C73}68,1 &
  \cellcolor[HTML]{E67C73}70,3 &
  \cellcolor[HTML]{E67C73}60,0 &
  \cellcolor[HTML]{E67C73}55,2 &
  \cellcolor[HTML]{E67C73}68,7 &
  \cellcolor[HTML]{E67C73}76,2 &
   &
   &
  F18 &
  \cellcolor[HTML]{E67C73}81,0 &
  \cellcolor[HTML]{E67C73}82,2 &
  \cellcolor[HTML]{E67C73}79,2 &
  \cellcolor[HTML]{E67C73}73,7 &
  \cellcolor[HTML]{E67C73}69,2 &
  \cellcolor[HTML]{E67C73}73,8 &
  \cellcolor[HTML]{E67C73}77,1 &
  \cellcolor[HTML]{E67C73}76,5 &
  \cellcolor[HTML]{DDD06E}31,2 &
  \cellcolor[HTML]{D5CF6F}29,5 &
  \cellcolor[HTML]{F8BA6A}42,3 &
  \cellcolor[HTML]{BFCB74}24,3 &
  \cellcolor[HTML]{EF9B6E}46,3 &
  \cellcolor[HTML]{FAD567}37,8 &
  \cellcolor[HTML]{EBD26B}34,4 &
  \cellcolor[HTML]{CACD72}26,8 \\ \cline{2-18} \cline{21-37} 
\multirow{-3}{*}{A08} &
  F17 &
  \cellcolor[HTML]{90C47E}14,7 &
  \cellcolor[HTML]{8BC37F}13,6 &
  \cellcolor[HTML]{94C47D}15,8 &
  \cellcolor[HTML]{A8C879}20,5 &
  \cellcolor[HTML]{A5C77A}20,0 &
  \cellcolor[HTML]{A3C77A}19,3 &
  \cellcolor[HTML]{8FC47E}14,6 &
  \cellcolor[HTML]{A6C779}20,2 &
  \cellcolor[HTML]{E67C73}62,0 &
  \cellcolor[HTML]{E67C73}63,8 &
  \cellcolor[HTML]{E67C73}58,3 &
  \cellcolor[HTML]{E67C73}75,6 &
  \cellcolor[HTML]{E67C73}52,8 &
  \cellcolor[HTML]{E67C73}64,4 &
  \cellcolor[HTML]{E67C73}65,2 &
  \cellcolor[HTML]{E67C73}65,5 &
   &
  \multirow{-3}{*}{A16} &
  F20 &
  \cellcolor[HTML]{E67C73}82,8 &
  \cellcolor[HTML]{E67C73}82,8 &
  \cellcolor[HTML]{E67C73}81,2 &
  \cellcolor[HTML]{E67C73}71,8 &
  \cellcolor[HTML]{E67C73}63,9 &
  \cellcolor[HTML]{E67C73}69,1 &
  \cellcolor[HTML]{E67C73}80,1 &
  \cellcolor[HTML]{E67C73}82,3 &
  \cellcolor[HTML]{B6CA76}22,3 &
  \cellcolor[HTML]{B0C977}21,0 &
  \cellcolor[HTML]{DBD06E}30,8 &
  \cellcolor[HTML]{D4CF70}29,1 &
  \cellcolor[HTML]{FFD366}39,2 &
  \cellcolor[HTML]{84C281}11,0 &
  \cellcolor[HTML]{E3D16C}32,5 &
  \cellcolor[HTML]{CCCD71}27,3 \\ \cline{1-18} \cline{20-37} 
\end{tabular}%
}
\caption{Top 3 features table}
\label{tab:3feat-table}
\end{table}
